Broken Neural Scaling Laws

We present a smoothly broken power law functional form (that we refer to as a Broken Neural Scaling Law (BNSL)) that accurately models & extrapolates the scaling behaviors of deep neural networks (i.e. how the evaluation metric of interest varies as amount of compute used for training (or inference), number of model parameters, training dataset size, model input size, number of training steps, or upstream performance varies) for various architectures & for each of various tasks within a large & diverse set of upstream & downstream tasks, in zero-shot, prompted, & finetuned settings. This set includes large-scale vision, language, audio, video, diffusion, generative modeling, multimodal learning, contrastive learning, AI alignment, AI capabilities, robotics, out-of-distribution (OOD) generalization, continual learning, transfer learning, uncertainty estimation / calibration, OOD detection, adversarial robustness, distillation, sparsity, retrieval, quantization, pruning, fairness, molecules, computer programming/coding, math word problems, "emergent phase transitions", arithmetic, supervised learning, unsupervised/self-supervised learning, & reinforcement learning (single agent & multi-agent). When compared to other functional forms for neural scaling, this functional form yields extrapolations of scaling behavior that are considerably more accurate on this set. Moreover, this functional form accurately models & extrapolates scaling behavior that other functional forms are incapable of expressing such as the nonmonotonic transitions present in the scaling behavior of phenomena such as double descent & the delayed, sharp inflection points present in the scaling behavior of tasks such as arithmetic. Lastly, we use this functional form to glean insights about the limit of the predictability of scaling behavior. Code is available at https://github.com/ethancaballero/broken_neural_scaling_laws

==> old__not_used_anymore/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> old__not_used_anymore/sections_ir/sec_bnsl_form.tex <==
\section{Proposed Functional Form: Broken Neural Scaling Laws }
\label{sec:bnsl}
\vspace{-0.08in}
The general functional form of a broken neural scaling law (BNSL) is given as follows:
%\begin{equation}
%y = \left(\frac{a}{x}\right)^b \left(1 + %\left(\frac{x}{c}\right)^d\right)^{-f} + g
%\label{eq:UniversalScalingLaw}
%\end{equation}
% \begin{equation}
% y = \left(\frac{a}{x}\right)^b \left(1 + \left(\frac{x}{c}\right)^d\right)^{-f} \left(1 + \left(\frac{x}{c}\right)^d\right)^{-f} + g
% \label{eq:UniversalScalingLaw}
% \end{equation}
%\todo[inline]{ How to best communicate that elements of equation 1 are added and removed based on number of breaks (see below)}
\begin{equation}
\vspace{-0.07in}
y =  a + \left(\frac{b}{x}\right)^c \prod_{i=1}^n \left(1 + \left(\frac{x}{d_i}\right)^{f_i}\right)^{-g_i},
\label{eq:UniversalScalingLaw}
\vspace{-0.07in}
\end{equation}
\begin{comment}
\iffalse
When $a = 0$, applying logarithms to both sides yields:
\begin{equation}
\log (y) =  c \log (b) - c \log(x) -  \sum_{i=1}^n g_i \log\left(1 + \left(\frac{x}{d_i}\right)^{f_i}\right).
%\label{eq:UniversalScalingLaw}
\end{equation}
TODO: I (David) made the above to try and get more intuition on this.  I guess it's not actually piece-wise linear (hence the SMOOTHLY broken)?
\fi
\end{comment}
%\begin{equation}
%y =  a + b^{-c} \prod_{i=1}^n \left(1 + {d_i}{x}^{-f_i}\right)^{-g_i}
%\label{eq:UniversalScalingLaw}
%\end{equation}
%In equation \ref{eq:UniversalScalingLaw}, 
where $y$ represents the performance evaluation metric (e.g. prediction error, cross entropy, BLEU score percentage, F1 score percentage, reward, or Elo rating) and $x$ represent whatever quantity is being scaled (e.g. number of model parameters, amount of compute used for training, or training dataset size). The variables $a, b, c, d_1 ...  d_n, f_1 ... f_n, g_1 ... g_n$ are all constants that are fit via curve fitting libraries such as SciPy \cite{virtanen2020scipy}.

The variable $n$ represents the number of breaks in the functional form, for a total of $n+1$ (approximately) linear regions on a log-log plot. A ``break" is defined as a transition between one interval that forms a straight line on a log-log plot and another interval that forms a straight line on a log-log plot.
The graph of this function (in a log-log plot) is not strictly speaking piece-wise linear; instead it smoothly interpolates between the different (approximately) linear regions. TODO: say something about why that is good.
%Most of our experiments use $n=1$, but we also show that 


%TODO: explain that there are varying number of variables $d_i, f_i, g_i$ depending on the number of breaks in the functional form.

Variable $a$ represents the limit as to how far the value of $y$ (performance evaluation metric) can be reduced (or maximized) as x (whatever quantity is being scaled) goes to infinity. Variable $b$ represents the offset of functional form on a log-log plot (analogous to $b$ in $y=mx+b$ on a linear-linear plot). Variable $c$ represents the slope of the first linear region on a log-log plot. Variable $d_i$ represents where on the x-axis the break between the $(i)$th and the $(i+1)$th linear region (on a log-log plot) occurs. Variable $f_i$ represents the slope of the $(i+1)$th linear region on a log-log plot. Variable $g_i$ represents the sharpness of break between the $(i)$th and the $(i+1)$th linear region on a log-log plot.



%TODO: note that equation \ref{eq:UniversalScalingLaw} works fine for upstream scaling too; we just name paper downstream scaling to emphasize the scenarios (i.e. downstream scaling) in which all its terms become necessary.

%\be
%\label{eq:PowerLawPlusConstant}
%L(x) = L_\infty + \left( \frac{x_0}{x}  \right)^{\alpha_x} 
%\ee

% \todo[inline]{this paragraph goes elsewhere} 
% We show mathematically and empirically that previous functional forms are unable to express inflection points, and we show mathematically and empirically that our functional form is able to express inflection points.



%We show that the functional form $y=a+(b/(x+c))^d$ (equation 1) very accurately fits 75\% of downstream tasks from the GPT-3 arXiv paper.


%When the best fit of equation 1 converges to values of d much larger than 1, the functional form equation 1 seems to not be sufficient and will probably need to be replaced with a new functional form.

%We find that the functional form $y=a+(b/((1+h)^x+c))^d$ (equation 2) is capable of fitting a subset of the downstream tasks (the downstream tasks for which equation 1 converges to values of d much larger than 1). However, equation 2 is much harder to fit due to small changes in h drastically changing y.


\iffalse
\begin{figure*}[t!]
\centering
\includegraphics[width=1.0\columnwidth]{figures/inflection_points/Two_Digit_Addition_Zero-Shot_Zoom.png}
\includegraphics[width=1.0\columnwidth]{figures/inflection_points/Two_Digit_Addition_Zero-Shot.png}
\caption{
Black points are test errors at various model sizes (numbers of parameters). Red line is functional form from equation \ref{eq:UniversalScalingLaw} fit to the black points. Left figure is zoomed in version of right figure. Task is Downstream Two Digit Addition (Zero-Shot) from \citet{brown2020language}. %\citet{2020arXiv200514165B}. 
All plots axes are \textbf{linear-linear} (not log-log).
}
\label{fig:Inflection_Point_example}
\end{figure*}
\fi


\iffalse
Our downstream forecasts show that an infinitely large (simultaneously infinitely deep and infinitely wide) GPT trained using the same 300 billion tokens as GPT-3 does not surpass human performance on any downstream task when using the few-shot in-context learning methodology from GPT-3 paper.
The one exception is fake news generation, for which our downstream forecast shows that humans would rate news articles generated by the model to be better than human written news articles 54.37\% of the time.

We perform ablations on the number of points and supremum of the points used for the fitting the scaling law functional form. These ablations provide some intuitions for how much to trust our forecasts.
\fi



==> old__not_used_anymore/sections_ir/sec_conclusions.tex <==
\section{Conclusions}
\noindent{\bf Summary.}

(TODO: This is just the abstract copied; and Surya's

We have presented a smoothly broken power law functional form that accurately models the scaling behaviors (of artificial neural networks) (i.e. how the evaluation metric of interest varies as the amount of compute used for training, number of model parameters, or training dataset size varies) for each task from a very large and diverse set of upstream and downstream (i.e. zero-shot, prompted, and fine-tuned) tasks. These tasks include large-scale vision tasks, large-scale unsupervised language tasks, arithmetic, and reinforcement learning. This functional form yields extrapolations of scaling behavior that often are an order of magnitude more accurate than other functional forms for modeling the scaling behavior of artificial neural networks. Furthermore, this functional form accurately models many scaling behaviors that other functional are mathematically incapable of expressing such as the non-monotonic transitions present in the scaling behavior of phenomena such as double descent and the delayed, sharp inflection points present in the scaling behavior of tasks such as arithmetic.

\noindent{\bf Limitations.} The most notable limitation   

\noindent{\bf Ethical considerations.} A potential negative societal impact could be that  

\noindent{\bf Future work.}
 

==> old__not_used_anymore/sections_ir/sec_experiments.tex <==
\section{Functional Form Fits and Extrapolations}
\label{section:functional_form_fits}

We now show the fits and/or extrapolations of various functional forms. In all plots here and in the appendix, black points are the points used for fitting a functional form, green points are the held-out points used for evaluating extrapolation of a functional form fit to the black points, and a red line is the BNSL that has been fit to the black points.

In the tables and elsewhere, 
\begin{itemize}
    \item M1 refers to functional form $y = ax^b$
    \item M2 refers to functional form $y = ax^b +c$
    \item M3 refers to functional form $y = a(x^{-1} + d)^{-b} + c$
    \item M4 refers to functional form $(y - \epsilon_{\infty}) / ((\epsilon_{0} - y)^a) = bx$
\end{itemize}

All the extrapolation evaluations reported in the tables are reported in terms of root mean squared log error (RMSLE\footnote{RMSLE = $ \sqrt{(\sum_{i=1}^{n} (log(y_{i})-log(\hat{y}_{i}))^2)/n}$}) ± root standard log error. 

TODO: define root standard log error; see commented out lines for how it's calculated
\[error = (log(y_{i})-log(\hat{y}_{i}))^2)\] 
\[\mu_{error} = \frac{1}{N}\sum_{i=1}^N error\]
\[\sigma_{error} = \sqrt{\frac{1}{N-1}\sum_{i=1}^N(error_i-\mu_{error})^2}\]
\[rstderr = \sqrt{\mu_{error} + \frac{\sigma_{error}}{\sqrt{len(\hat{y})}}} - \sqrt{\mu_{error}}\] 
% how root standard log error is calculated
%error = (np.log(yp) - np.log(y)) ** 2
%errmu = np.mean(error)
%rstderr = np.sqrt(errmu + np.std(error) / (len(yp)**0.5)) - np.sqrt(errmu)

\FloatBarrier
\subsection{Vision}
\label{section:scaling_benchmark__vision}

(TODO: this sentence is repeated in language section)

Using the scaling laws benchmark of \cite{Alabdulmohsi2022revisiting}, we evaluate how well various functional forms extrapolate performance on vision tasks as training dataset size increases. In this vision subset of the benchmark, the tasks that are evaluated are error rate on each of various few-shot downstream image classification (IC) tasks; the downstream tasks are: Birds 200 \cite{welinder2010caltech}, Caltech101 \cite{fei2004learning}, CIFAR-100 \cite{krizhevsky2009learning}, and ImageNet \cite{deng2009imagenet}. The following architectures of various sizes are pretrained on subsets of JFT-300M: big-transfer residual neural networks (BiT) \cite{kolesnikov2020big}, MLP mixers (MiX) \cite{tolstikhin2021mlp}, and vision transformers (ViT) \cite{dosovitskiy2020image}. As can be seen in Table  \ref{table:scaling_laws_benchmark_dataset__Vision}, BNSL (TODO: make sure BNSL abbreviation is defined somewhere) yields extrapolations with the lowest RMSLE (Root Mean Squared Logarithmic Error) for the largest number (by a very large margin) (TODO: replace "large margin" with numbers) of tasks of any of the functional forms.

To view all plots of the BNSL on each of these tasks, see figures
\ref{fig:scaling_laws_benchmark_dataset__birds},
\ref{fig:scaling_laws_benchmark_dataset__cifar_100},
\ref{fig:scaling_laws_benchmark_dataset__caltech},
\ref{fig:scaling_laws_benchmark_dataset__ImageNet} in Appendix \ref{section:Plots_of_BNSL_Extrapolations}. To view all plots of M1, M2, M3, and M4 on each of these tasks, see Appendix A.4 of \cite{Alabdulmohsi2022revisiting}.

% \begin{center}
\begin{table}
    \centering
    \begin{tabular}{ |c|c|c|c|c|c|c| } 
\hline
Domain & \hspace{.9cm}Task & M1 $\uparrow$ & M2 $\uparrow$ & M3 $\uparrow$ & M4 $\uparrow$ & BNSL $\uparrow$ \\
 \hline
 IC & Birds 200 & 0 & 0 & 0 & 5.56 & \highlight{94.44}\\ 
 IC & Caltech101 & 0 & 0 & 5.56 & 5.56 & \highlight{88.89}\\ 
 IC & CIFAR-100 & 0 & 5.56 & 5.56 & 5.56 & \highlight{83.33}\\
 IC & ImageNet & 0 & 0 & 11.11 & 0 & \highlight{88.89}\\
 Language & All & 5 & 10 & 15 & 25 & \highlight{45}\\
 \hline
\end{tabular}
    \caption{
    Percentage of tasks by domain where each functional form is the best for extrapolation. See Section \ref{section:scaling_benchmark__vision} for more details. Numbers for M1, M2, M3, and M4 were obtained via correspondence with authors of \cite{Alabdulmohsi2022revisiting}. 
    }
    \label{table:scaling_laws_benchmark_dataset__Vision}
\end{table}
% \end{center}

\begin{table}[htbp]
\tiny
% \fontsize{8}{8}\selectfont
% \setlength\tabcolsep{3.1pt} 
\begin{tabular}
%{p{.02\textwidth}p{.165\textwidth}p{.095\textwidth}p{.01\textwidth}p{.01\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}}
{p{.205\textwidth}p{.111\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}}
%\begin{tabular}{llllrrrrrrrrrrrrl}
\hspace{.9cm}Task & Model & M1 $\downarrow$ & M2 $\downarrow$ & M3 $\downarrow$ & M4 $\downarrow$ & BNSL $\downarrow$ \\
\hline
Birds 200 10-shot & BiT/101/3 & 9.13e-2 & 9.13e-2 & 9.13e-2 & 2.49e-2 & \highlight{3.79e-3} \\
Birds 200 10-shot & BiT/50/1 & 6.88e-2 & 6.88e-2 & 5.24e-2 & 2.48e-2 & \highlight{4.96e-3} \\
Birds 200 10-shot & MiX/B/16 & 9.15e-2 & 9.15e-2 & 3.95e-2 & 4.14e-2 & \highlight{9.98e-3} \\
Birds 200 10-shot & MiX/L/16 & 5.51e-2 & 5.51e-2 & 5.51e-2 & 4.59e-2 & \highlight{8.41e-3} \\
Birds 200 10-shot & ViT/B/16 & 6.77e-2 & 6.77e-2 & 3.52e-2 & 1.87e-2 & \highlight{9.81e-3} \\
Birds 200 10-shot & ViT/S/16 & 3.95e-2 & 3.95e-2 & 3.74e-2 & \highlight{9.81e-3} & 1.51e-2 \\
Birds 200 25-shot & BiT/101/3 & 9.41e-2 & 9.41e-2 & 9.41e-2 & 5.09e-2 & \highlight{7.24e-3} \\
Birds 200 25-shot & BiT/50/1 & 1.10e-1 & 7.29e-2 & 1.52e-2 & 1.63e-2 & \highlight{8.00e-3} \\
Birds 200 25-shot & MiX/B/16 & 1.40e-1 & 1.40e-1 & 6.93e-2 & 1.85e-2 & \highlight{5.02e-3} \\
Birds 200 25-shot & MiX/L/16 & 1.12e-1 & 1.12e-1 & 1.12e-1 & 4.88e-2 & \highlight{1.05e-2} \\
Birds 200 25-shot & ViT/B/16 & 9.02e-2 & 9.02e-2 & 3.75e-2 & 1.52e-2 & \highlight{5.87e-3} \\
Birds 200 25-shot & ViT/S/16 & 5.06e-2 & 5.06e-2 & 4.96e-2 & 3.28e-2 & \highlight{1.21e-2} \\
Birds 200 5-shot & BiT/101/3 & 8.17e-2 & 8.17e-2 & 8.17e-2 & 3.00e-2 & \highlight{6.08e-3} \\
Birds 200 5-shot & BiT/50/1 & 5.44e-2 & 5.44e-2 & 5.44e-2 & 2.63e-2 & \highlight{5.79e-3} \\
Birds 200 5-shot & MiX/B/16 & 8.27e-2 & 8.27e-2 & 5.49e-2 & 1.86e-2 & \highlight{5.74e-3} \\
Birds 200 5-shot & MiX/L/16 & 5.68e-2 & 5.68e-2 & 5.68e-2 & 2.65e-2 & \highlight{5.06e-3} \\
Birds 200 5-shot & ViT/B/16 & 3.40e-2 & 3.40e-2 & 3.40e-2 & 1.26e-2 & \highlight{6.32e-3} \\
Birds 200 5-shot & ViT/S/16 & 2.75e-2 & 2.75e-2 & 2.75e-2 & 1.56e-2 & \highlight{6.93e-3} \\
\hline
CIFAR-100 10-shot & BiT/101/3 & 8.57e-2 & 8.57e-2 & 8.25e-2 & 9.28e-2 & \highlight{1.53e-2} \\
CIFAR-100 10-shot & BiT/50/1 & 7.44e-2 & 1.24e-2 & 2.08e-2 & 1.23e-2 & \highlight{9.74e-3} \\
CIFAR-100 10-shot & MiX/B/16 & 8.77e-2 & 8.77e-2 & 2.71e-2 & 2.60e-2 & \highlight{8.61e-3} \\
CIFAR-100 10-shot & MiX/L/16 & 1.05e-1 & 1.05e-1 & 4.85e-2 & 4.76e-2 & \highlight{1.55e-2} \\
CIFAR-100 10-shot & ViT/B/16 & 8.98e-2 & 8.98e-2 & 8.98e-2 & 5.60e-2 & \highlight{1.73e-2} \\
CIFAR-100 10-shot & ViT/S/16 & 6.84e-2 & 2.11e-2 & 3.35e-2 & 2.47e-2 & \highlight{1.15e-2} \\
CIFAR-100 25-shot & BiT/101/3 & 8.77e-2 & 8.77e-2 & 4.44e-2 & 4.29e-2 & \highlight{9.32e-3} \\
CIFAR-100 25-shot & BiT/50/1 & 7.31e-2 & 2.35e-2 & 3.65e-2 & 2.36e-2 & \highlight{2.00e-2} \\
CIFAR-100 25-shot & MiX/B/16 & 1.08e-1 & 4.75e-2 & 2.10e-2 & 2.08e-2 & \highlight{8.15e-3} \\
CIFAR-100 25-shot & MiX/L/16 & 9.79e-2 & 9.79e-2 & 3.67e-2 & 2.79e-2 & \highlight{8.47e-3} \\
CIFAR-100 25-shot & ViT/B/16 & 1.07e-1 & 1.07e-1 & 6.54e-2 & \highlight{4.81e-2} & 1.20e-1 \\
CIFAR-100 25-shot & ViT/S/16 & 8.03e-2 & 2.19e-2 & 3.13e-2 & 2.19e-2 & \highlight{1.34e-2} \\
CIFAR-100 5-shot & BiT/101/3 & 5.94e-2 & 5.94e-2 & 5.94e-2 & 4.57e-2 & \highlight{1.58e-2} \\
CIFAR-100 5-shot & BiT/50/1 & 4.87e-2 & 4.87e-2 & \highlight{1.69e-2} & 4.91e-2 & 1.95e-2 \\
CIFAR-100 5-shot & MiX/B/16 & 7.07e-2 & 7.07e-2 & 2.78e-2 & 2.05e-2 & \highlight{6.77e-3} \\
CIFAR-100 5-shot & MiX/L/16 & 7.06e-2 & 7.06e-2 & 4.17e-2 & 3.14e-2 & \highlight{1.18e-2} \\
CIFAR-100 5-shot & ViT/B/16 & 6.27e-2 & 6.27e-2 & 6.27e-2 & 5.11e-2 & \highlight{1.19e-2} \\
CIFAR-100 5-shot & ViT/S/16 & 6.93e-2 & \highlight{2.84e-2} & 3.88e-2 & 3.09e-2 & 6.40e-2 \\
\hline
Caltech101 10-shot & BiT/101/3 & 3.07e-1 & 3.07e-1 & 1.51e-1 & 3.54e-2 & \highlight{6.42e-3} \\
Caltech101 10-shot & BiT/50/1 & 3.29e-1 & 7.68e-2 & 1.13e-1 & 6.31e-2 & \highlight{5.37e-3} \\
Caltech101 10-shot & MiX/B/16 & 1.35e-1 & 1.35e-1 & 1.35e-1 & 2.11e-1 & \highlight{3.72e-2} \\
Caltech101 10-shot & MiX/L/16 & 1.25e-1 & 1.25e-1 & 1.25e-1 & 1.92e-1 & \highlight{3.73e-2} \\
Caltech101 10-shot & ViT/B/16 & 7.76e-2 & 7.76e-2 & 3.11e-2 & 5.54e-2 & \highlight{1.67e-2} \\
Caltech101 10-shot & ViT/S/16 & 1.95e-1 & 3.41e-2 & \highlight{2.40e-2} & 3.95e-2 & 3.31e-2 \\
Caltech101 25-shot & BiT/101/3 & 1.15e-1 & 1.15e-1 & 1.15e-1 & 5.23e-2 & \highlight{1.13e-2} \\
Caltech101 25-shot & BiT/50/1 & 3.60e-1 & 8.80e-2 & 1.43e-1 & 5.95e-2 & \highlight{2.13e-3} \\
Caltech101 25-shot & MiX/B/16 & 8.28e-2 & 8.28e-2 & 8.28e-2 & 1.74e-1 & \highlight{2.83e-2} \\
Caltech101 25-shot & MiX/L/16 & 9.66e-2 & 9.66e-2 & 9.66e-2 & 1.03e-1 & \highlight{1.98e-2} \\
Caltech101 25-shot & ViT/B/16 & 1.03e-1 & 3.33e-2 & 4.46e-2 & 4.24e-2 & \highlight{6.37e-3} \\
Caltech101 25-shot & ViT/S/16 & 1.77e-1 & 3.79e-2 & 2.80e-2 & \highlight{2.35e-2} & 2.38e-2 \\
Caltech101 5-shot & BiT/101/3 & 2.12e-1 & 2.12e-1 & 2.12e-1 & 8.82e-2 & \highlight{3.17e-3} \\
Caltech101 5-shot & BiT/50/1 & 2.34e-1 & 4.13e-2 & 1.61e-2 & 4.49e-2 & \highlight{1.33e-2} \\
Caltech101 5-shot & MiX/B/16 & 2.43e-1 & 2.43e-1 & 2.35e-1 & 1.23e-1 & \highlight{3.59e-3} \\
Caltech101 5-shot & MiX/L/16 & 1.38e-1 & 1.38e-1 & 1.38e-1 & 3.19e-2 & \highlight{3.19e-2} \\
Caltech101 5-shot & ViT/B/16 & 1.10e-1 & 1.10e-1 & 6.02e-2 & 6.59e-2 & \highlight{2.33e-2} \\
Caltech101 5-shot & ViT/S/16 & 1.90e-1 & 3.82e-2 & 5.04e-2 & 4.06e-2 & \highlight{2.47e-2} \\
\hline
ImageNet 10-shot & BiT/101/3 & 1.27e-1 & 1.27e-1 & 7.36e-2 & 2.13e-2 & \highlight{5.95e-3} \\
ImageNet 10-shot & BiT/50/1 & 9.54e-2 & 9.54e-2 & \highlight{5.75e-3} & 1.77e-2 & 8.93e-3 \\
ImageNet 10-shot & MiX/B/16 & 9.34e-2 & 9.34e-2 & 3.37e-2 & 1.80e-2 & \highlight{5.88e-3} \\
ImageNet 10-shot & MiX/L/16 & 9.83e-2 & 9.83e-2 & 9.83e-2 & 9.48e-3 & \highlight{3.81e-3} \\
ImageNet 10-shot & ViT/B/16 & 4.62e-2 & 4.62e-2 & 4.62e-2 & 3.43e-2 & \highlight{2.85e-3} \\
ImageNet 10-shot & ViT/S/16 & 4.74e-2 & 4.74e-2 & 1.66e-2 & 1.14e-2 & \highlight{1.97e-3} \\
ImageNet 25-shot & BiT/101/3 & 1.42e-1 & 1.42e-1 & 6.67e-2 & 2.18e-2 & \highlight{4.86e-3} \\
ImageNet 25-shot & BiT/50/1 & 1.17e-1 & 1.17e-1 & \highlight{4.06e-3} & 1.70e-2 & 8.14e-3 \\
ImageNet 25-shot & MiX/B/16 & 9.59e-2 & 9.59e-2 & 5.39e-2 & 1.47e-2 & \highlight{2.86e-3} \\
ImageNet 25-shot & MiX/L/16 & 1.03e-1 & 1.03e-1 & 1.03e-1 & 6.09e-3 & \highlight{1.94e-3} \\
ImageNet 25-shot & ViT/B/16 & 5.17e-2 & 5.17e-2 & 5.17e-2 & 3.26e-2 & \highlight{6.91e-3} \\
ImageNet 25-shot & ViT/S/16 & 5.52e-2 & 4.12e-2 & 9.65e-3 & 1.16e-2 & \highlight{3.09e-3} \\
ImageNet 5-shot & BiT/101/3 & 9.24e-2 & 9.24e-2 & 9.24e-2 & 1.01e-2 & \highlight{2.55e-3} \\
ImageNet 5-shot & BiT/50/1 & 8.95e-2 & 8.95e-2 & 1.53e-2 & 1.03e-2 & \highlight{4.00e-3} \\
ImageNet 5-shot & MiX/B/16 & 9.09e-2 & 9.09e-2 & 3.01e-2 & 1.45e-2 & \highlight{3.57e-3} \\
ImageNet 5-shot & MiX/L/16 & 7.99e-2 & 7.99e-2 & 7.99e-2 & 5.66e-3 & \highlight{1.63e-3} \\
ImageNet 5-shot & ViT/B/16 & 4.11e-2 & 4.11e-2 & 4.11e-2 & 2.88e-2 & \highlight{4.97e-3} \\
ImageNet 5-shot & ViT/S/16 & 4.20e-2 & 4.20e-2 & 2.40e-2 & 1.44e-2 & \highlight{3.00e-3} \\
\end{tabular}
    \caption{
    Extrapolation Results for Vision Tasks. See Section \ref{section:scaling_benchmark__vision} for more details. Numbers for M1, M2, M3, and M4 obtained via correspondence with authors of \cite{Alabdulmohsi2022revisiting}. 
    }
    \label{table:scaling_laws_benchmark_dataset__Vision}
\end{table}
\FloatBarrier

\begin{table}[htbp]
\begin{adjustwidth}{-2.2cm}{-1cm}
\fontsize{8}{10}\selectfont
% \setlength\tabcolsep{3.1pt} 
\begin{tabular}
{|p{.165\textwidth} c c c c c || p{.165\textwidth} c c c c c |}
%{p{.02\textwidth}p{.165\textwidth}p{.095\textwidth}p{.01\textwidth}p{.01\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}}
% {p{.165\textwidth}p{.070\textwidth}p{.070\textwidth}p{.080\textwidth}p{.080\textwidth}p{.080\textwidth}p{.165\textwidth}p{.080\textwidth}p{.080\textwidth}p{.080\textwidth}p{.080\textwidth}p{.080\textwidth}}
%\begin{tabular}{llllrrrrrrrrrrrrl}
\hline
\hspace{.9cm}Task & M1 $\downarrow$ & M2 $\downarrow$ & M3 $\downarrow$ & M4 $\downarrow$ & BNSL $\downarrow$ & \hspace{.9cm}Task & M1 $\downarrow$ & M2 $\downarrow$ & M3 $\downarrow$ & M4 $\downarrow$ & BNSL $\downarrow$\\
\hline
Birds 200 10-shot & 9.13e-2 & 9.13e-2 & 9.13e-2 & 2.49e-2 & \highlight{3.79e-3} & CIFAR-100 10-shot & 8.57e-2 & 8.57e-2 & 8.25e-2 & 9.28e-2 & \highlight{1.53e-2} \\
Birds 200 10-shot & 6.88e-2 & 6.88e-2 & 5.24e-2 & 2.48e-2 & \highlight{4.96e-3} & CIFAR-100 10-shot & 7.44e-2 & 1.24e-2 & 2.08e-2 & 1.23e-2 & \highlight{9.74e-3} \\
Birds 200 10-shot & 9.15e-2 & 9.15e-2 & 3.95e-2 & 4.14e-2 & \highlight{9.98e-3} & CIFAR-100 10-shot & 8.77e-2 & 8.77e-2 & 2.71e-2 & 2.60e-2 & \highlight{8.61e-3} \\
Birds 200 10-shot & 5.51e-2 & 5.51e-2 & 5.51e-2 & 4.59e-2 & \highlight{8.41e-3} & CIFAR-100 10-shot & 1.05e-1 & 1.05e-1 & 4.85e-2 & 4.76e-2 & \highlight{1.55e-2} \\
Birds 200 10-shot & 6.77e-2 & 6.77e-2 & 3.52e-2 & 1.87e-2 & \highlight{9.81e-3} & CIFAR-100 10-shot & 8.98e-2 & 8.98e-2 & 8.98e-2 & 5.60e-2 & \highlight{1.73e-2} \\
Birds 200 10-shot & 3.95e-2 & 3.95e-2 & 3.74e-2 & \highlight{9.81e-3} & 1.51e-2 & CIFAR-100 10-shot & 6.84e-2 & 2.11e-2 & 3.35e-2 & 2.47e-2 & \highlight{1.15e-2} \\
Birds 200 25-shot & 9.41e-2 & 9.41e-2 & 9.41e-2 & 5.09e-2 & \highlight{7.24e-3} & CIFAR-100 25-shot & 8.77e-2 & 8.77e-2 & 4.44e-2 & 4.29e-2 & \highlight{9.32e-3} \\
Birds 200 25-shot & 1.10e-1 & 7.29e-2 & 1.52e-2 & 1.63e-2 & \highlight{8.00e-3} & CIFAR-100 25-shot & 7.31e-2 & 2.35e-2 & 3.65e-2 & 2.36e-2 & \highlight{2.00e-2} \\
Birds 200 25-shot & 1.40e-1 & 1.40e-1 & 6.93e-2 & 1.85e-2 & \highlight{5.02e-3} & CIFAR-100 25-shot & 1.08e-1 & 4.75e-2 & 2.10e-2 & 2.08e-2 & \highlight{8.15e-3} \\
Birds 200 25-shot & 1.12e-1 & 1.12e-1 & 1.12e-1 & 4.88e-2 & \highlight{1.05e-2} & CIFAR-100 25-shot & 9.79e-2 & 9.79e-2 & 3.67e-2 & 2.79e-2 & \highlight{8.47e-3} \\
Birds 200 25-shot & 9.02e-2 & 9.02e-2 & 3.75e-2 & 1.52e-2 & \highlight{5.87e-3} & CIFAR-100 25-shot & 1.07e-1 & 1.07e-1 & 6.54e-2 & \highlight{4.81e-2} & 1.20e-1 \\
Birds 200 25-shot & 5.06e-2 & 5.06e-2 & 4.96e-2 & 3.28e-2 & \highlight{1.21e-2} & CIFAR-100 25-shot & 8.03e-2 & 2.19e-2 & 3.13e-2 & 2.19e-2 & \highlight{1.34e-2} \\
Birds 200 5-shot & 8.17e-2 & 8.17e-2 & 8.17e-2 & 3.00e-2 & \highlight{6.08e-3} & CIFAR-100 5-shot & 5.94e-2 & 5.94e-2 & 5.94e-2 & 4.57e-2 & \highlight{1.58e-2} \\
Birds 200 5-shot & 5.44e-2 & 5.44e-2 & 5.44e-2 & 2.63e-2 & \highlight{5.79e-3} & CIFAR-100 5-shot & 4.87e-2 & 4.87e-2 & \highlight{1.69e-2} & 4.91e-2 & 1.95e-2 \\
Birds 200 5-shot & 8.27e-2 & 8.27e-2 & 5.49e-2 & 1.86e-2 & \highlight{5.74e-3} & CIFAR-100 5-shot & 7.07e-2 & 7.07e-2 & 2.78e-2 & 2.05e-2 & \highlight{6.77e-3} \\
Birds 200 5-shot & 5.68e-2 & 5.68e-2 & 5.68e-2 & 2.65e-2 & \highlight{5.06e-3} & CIFAR-100 5-shot & 7.06e-2 & 7.06e-2 & 4.17e-2 & 3.14e-2 & \highlight{1.18e-2} \\
Birds 200 5-shot & 3.40e-2 & 3.40e-2 & 3.40e-2 & 1.26e-2 & \highlight{6.32e-3} & CIFAR-100 5-shot & 6.27e-2 & 6.27e-2 & 6.27e-2 & 5.11e-2 & \highlight{1.19e-2} \\
Birds 200 5-shot & 2.75e-2 & 2.75e-2 & 2.75e-2 & 1.56e-2 & \highlight{6.93e-3} & CIFAR-100 5-shot & 6.93e-2 & \highlight{2.84e-2} & 3.88e-2 & 3.09e-2 & 6.40e-2 \\
\hline
\hline
Caltech101 10-shot & 3.07e-1 & 3.07e-1 & 1.51e-1 & 3.54e-2 & \highlight{6.42e-3} & ImageNet 10-shot & 1.27e-1 & 1.27e-1 & 7.36e-2 & 2.13e-2 & \highlight{5.95e-3} \\
Caltech101 10-shot & 3.29e-1 & 7.68e-2 & 1.13e-1 & 6.31e-2 & \highlight{5.37e-3} & ImageNet 10-shot & 9.54e-2 & 9.54e-2 & \highlight{5.75e-3} & 1.77e-2 & 8.93e-3 \\
Caltech101 10-shot & 1.35e-1 & 1.35e-1 & 1.35e-1 & 2.11e-1 & \highlight{3.72e-2} & ImageNet 10-shot & 9.34e-2 & 9.34e-2 & 3.37e-2 & 1.80e-2 & \highlight{5.88e-3} \\
Caltech101 10-shot & 1.25e-1 & 1.25e-1 & 1.25e-1 & 1.92e-1 & \highlight{3.73e-2} & ImageNet 10-shot & 9.83e-2 & 9.83e-2 & 9.83e-2 & 9.48e-3 & \highlight{3.81e-3} \\
Caltech101 10-shot & 7.76e-2 & 7.76e-2 & 3.11e-2 & 5.54e-2 & \highlight{1.67e-2} & ImageNet 10-shot & 4.62e-2 & 4.62e-2 & 4.62e-2 & 3.43e-2 & \highlight{2.85e-3} \\
Caltech101 10-shot & 1.95e-1 & 3.41e-2 & \highlight{2.40e-2} & 3.95e-2 & 3.31e-2 & ImageNet 10-shot & 4.74e-2 & 4.74e-2 & 1.66e-2 & 1.14e-2 & \highlight{1.97e-3} \\
Caltech101 25-shot & 1.15e-1 & 1.15e-1 & 1.15e-1 & 5.23e-2 & \highlight{1.13e-2} & ImageNet 25-shot & 1.42e-1 & 1.42e-1 & 6.67e-2 & 2.18e-2 & \highlight{4.86e-3} \\
Caltech101 25-shot & 3.60e-1 & 8.80e-2 & 1.43e-1 & 5.95e-2 & \highlight{2.13e-3} & ImageNet 25-shot & 1.17e-1 & 1.17e-1 & \highlight{4.06e-3} & 1.70e-2 & 8.14e-3 \\
Caltech101 25-shot & 8.28e-2 & 8.28e-2 & 8.28e-2 & 1.74e-1 & \highlight{2.83e-2} & ImageNet 25-shot & 9.59e-2 & 9.59e-2 & 5.39e-2 & 1.47e-2 & \highlight{2.86e-3} \\
Caltech101 25-shot & 9.66e-2 & 9.66e-2 & 9.66e-2 & 1.03e-1 & \highlight{1.98e-2} & ImageNet 25-shot & 1.03e-1 & 1.03e-1 & 1.03e-1 & 6.09e-3 & \highlight{1.94e-3} \\
Caltech101 25-shot & 1.03e-1 & 3.33e-2 & 4.46e-2 & 4.24e-2 & \highlight{6.37e-3} & ImageNet 25-shot & 5.17e-2 & 5.17e-2 & 5.17e-2 & 3.26e-2 & \highlight{6.91e-3} \\
Caltech101 25-shot & 1.77e-1 & 3.79e-2 & 2.80e-2 & \highlight{2.35e-2} & 2.38e-2 & ImageNet 25-shot & 5.52e-2 & 4.12e-2 & 9.65e-3 & 1.16e-2 & \highlight{3.09e-3} \\
Caltech101 5-shot & 2.12e-1 & 2.12e-1 & 2.12e-1 & 8.82e-2 & \highlight{3.17e-3} & ImageNet 5-shot & 9.24e-2 & 9.24e-2 & 9.24e-2 & 1.01e-2 & \highlight{2.55e-3} \\
Caltech101 5-shot & 2.34e-1 & 4.13e-2 & 1.61e-2 & 4.49e-2 & \highlight{1.33e-2} & ImageNet 5-shot & 8.95e-2 & 8.95e-2 & 1.53e-2 & 1.03e-2 & \highlight{4.00e-3} \\
Caltech101 5-shot & 2.43e-1 & 2.43e-1 & 2.35e-1 & 1.23e-1 & \highlight{3.59e-3} & ImageNet 5-shot & 9.09e-2 & 9.09e-2 & 3.01e-2 & 1.45e-2 & \highlight{3.57e-3} \\
Caltech101 5-shot & 1.38e-1 & 1.38e-1 & 1.38e-1 & 3.19e-2 & \highlight{3.19e-2} & ImageNet 5-shot & 7.99e-2 & 7.99e-2 & 7.99e-2 & 5.66e-3 & \highlight{1.63e-3} \\
Caltech101 5-shot & 1.10e-1 & 1.10e-1 & 6.02e-2 & 6.59e-2 & \highlight{2.33e-2} & ImageNet 5-shot & 4.11e-2 & 4.11e-2 & 4.11e-2 & 2.88e-2 & \highlight{4.97e-3} \\
Caltech101 5-shot & 1.90e-1 & 3.82e-2 & 5.04e-2 & 4.06e-2 & \highlight{2.47e-2} & ImageNet 5-shot & 4.20e-2 & 4.20e-2 & 2.40e-2 & 1.44e-2 & \highlight{3.00e-3} \\
\hline
\end{tabular}
    \caption{
    Extrapolation Results for Vision Tasks. See Section \ref{section:scaling_benchmark__vision} for more details. Numbers for M1, M2, M3, and M4 obtained via correspondence with authors of \cite{Alabdulmohsi2022revisiting}. 
    }
    \label{table:scaling_laws_benchmark_dataset__Vision}
\end{adjustwidth}
\end{table}
\FloatBarrier

\begin{table}[htbp]
\tiny
\setlength\tabcolsep{3.1pt} 
\begin{tabular}
%{p{.02\textwidth}p{.165\textwidth}p{.095\textwidth}p{.01\textwidth}p{.01\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}}
{p{.021\textwidth}p{.165\textwidth}p{.111\textwidth}p{.028\textwidth}p{.022\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}}
%\begin{tabular}{llllrrrrrrrrrrrrl}
Domain & \hspace{.9cm}Task & Model & Train Points & Test Points & M1 $\downarrow$ & M2 $\downarrow$ & M3 $\downarrow$ & M4 $\downarrow$ & BNSL $\downarrow$ \\
\hline
IC & Birds 200 10-shot & BiT/101/3 & 57 & 107 & 9.13e-2 ± 2.8e-3 & 9.13e-2 ± 2.8e-3 & 9.13e-2 ± 2.8e-3 & 2.49e-2 ± 1.2e-3 & \bfseries 3.79e-3 ± 1.1e-3 \\
IC & Birds 200 10-shot & BiT/50/1 & 70 & 469 & 6.88e-2 ± 7.5e-4 & 6.88e-2 ± 7.5e-4 & 5.24e-2 ± 6.2e-4 & 2.48e-2 ± 5.1e-4 & \bfseries 4.96e-3 ± 3.9e-4 \\
IC & Birds 200 10-shot & MiX/B/16 & 69 & 383 & 9.15e-2 ± 1.1e-3 & 9.15e-2 ± 1.1e-3 & 3.95e-2 ± 7.0e-4 & 4.14e-2 ± 7.8e-4 & \bfseries 9.98e-3 ± 7.0e-4 \\
IC & Birds 200 10-shot & MiX/L/16 & 63 & 211 & 5.51e-2 ± 1.4e-3 & 5.51e-2 ± 1.4e-3 & 5.51e-2 ± 1.4e-3 & 4.59e-2 ± 1.6e-3 & \bfseries 8.41e-3 ± 1.3e-3 \\
IC & Birds 200 10-shot & ViT/B/16 & 65 & 316 & 6.77e-2 ± 1.1e-3 & 6.77e-2 ± 1.1e-3 & 3.52e-2 ± 8.1e-4 & 1.87e-2 ± 7.2e-4 & \bfseries 9.81e-3 ± 8.1e-4 \\
IC & Birds 200 10-shot & ViT/S/16 & 54 & 133 & 3.95e-2 ± 1.2e-3 & 3.95e-2 ± 1.2e-3 & 3.74e-2 ± 1.1e-3 & \bfseries 9.81e-3 ± 5.4e-4 & 1.51e-2 ± 8.4e-4 \\
IC & Birds 200 25-shot & BiT/101/3 & 53 & 78 & 9.41e-2 ± 3.2e-3 & 9.41e-2 ± 3.2e-3 & 9.41e-2 ± 3.2e-3 & 5.09e-2 ± 1.8e-3 & \bfseries 7.24e-3 ± 1.6e-3 \\
IC & Birds 200 25-shot & BiT/50/1 & 69 & 452 & 1.10e-1 ± 1.0e-3 & 7.29e-2 ± 8.0e-4 & 1.52e-2 ± 4.9e-4 & 1.63e-2 ± 5.1e-4 & \bfseries 8.00e-3 ± 6.1e-4 \\
IC & Birds 200 25-shot & MiX/B/16 & 67 & 293 & 1.40e-1 ± 1.9e-3 & 1.40e-1 ± 1.9e-3 & 6.93e-2 ± 1.2e-3 & 1.85e-2 ± 6.3e-4 & \bfseries 5.02e-3 ± 6.2e-4 \\
IC & Birds 200 25-shot & MiX/L/16 & 63 & 196 & 1.12e-1 ± 2.0e-3 & 1.12e-1 ± 2.0e-3 & 1.12e-1 ± 2.0e-3 & 4.88e-2 ± 1.8e-3 & \bfseries 1.05e-2 ± 1.7e-3 \\
IC & Birds 200 25-shot & ViT/B/16 & 64 & 271 & 9.02e-2 ± 1.6e-3 & 9.02e-2 ± 1.6e-3 & 3.75e-2 ± 1.0e-3 & 1.52e-2 ± 5.8e-4 & \bfseries 5.87e-3 ± 6.1e-4 \\
IC & Birds 200 25-shot & ViT/S/16 & 51 & 100 & 5.06e-2 ± 1.4e-3 & 5.06e-2 ± 1.4e-3 & 4.96e-2 ± 1.4e-3 & 3.28e-2 ± 1.1e-3 & \bfseries 1.21e-2 ± 8.5e-4 \\
IC & Birds 200 5-shot & BiT/101/3 & 62 & 180 & 8.17e-2 ± 2.0e-3 & 8.17e-2 ± 2.0e-3 & 8.17e-2 ± 2.0e-3 & 3.00e-2 ± 1.2e-3 & \bfseries 6.08e-3 ± 1.1e-3 \\
IC & Birds 200 5-shot & BiT/50/1 & 71 & 517 & 5.44e-2 ± 5.6e-4 & 5.44e-2 ± 5.6e-4 & 5.44e-2 ± 5.6e-4 & 2.63e-2 ± 5.4e-4 & \bfseries 5.79e-3 ± 3.7e-4 \\
IC & Birds 200 5-shot & MiX/B/16 & 71 & 494 & 8.27e-2 ± 1.0e-3 & 8.27e-2 ± 1.0e-3 & 5.49e-2 ± 7.8e-4 & 1.86e-2 ± 5.0e-4 & \bfseries 5.74e-3 ± 4.7e-4 \\
IC & Birds 200 5-shot & MiX/L/16 & 67 & 326 & 5.68e-2 ± 1.4e-3 & 5.68e-2 ± 1.4e-3 & 5.68e-2 ± 1.4e-3 & 2.65e-2 ± 9.0e-4 & \bfseries 5.06e-3 ± 6.4e-4 \\
IC & Birds 200 5-shot & ViT/B/16 & 65 & 284 & 3.40e-2 ± 8.9e-4 & 3.40e-2 ± 8.9e-4 & 3.40e-2 ± 8.9e-4 & 1.26e-2 ± 5.3e-4 & \bfseries 6.32e-3 ± 5.8e-4 \\
IC & Birds 200 5-shot & ViT/S/16 & 57 & 150 & 2.75e-2 ± 7.9e-4 & 2.75e-2 ± 7.9e-4 & 2.75e-2 ± 7.9e-4 & 1.56e-2 ± 5.9e-4 & \bfseries 6.93e-3 ± 4.8e-4 \\
IC & CIFAR-100 10-shot & BiT/101/3 & 47 & 60 & 8.57e-2 ± 3.8e-3 & 8.57e-2 ± 3.8e-3 & 8.25e-2 ± 3.7e-3 & 9.28e-2 ± 3.9e-3 & \bfseries 1.53e-2 ± 2.9e-3 \\
IC & CIFAR-100 10-shot & BiT/50/1 & 62 & 192 & 7.44e-2 ± 1.5e-3 & 1.24e-2 ± 5.8e-4 & 2.08e-2 ± 7.2e-4 & 1.23e-2 ± 5.7e-4 & \bfseries 9.74e-3 ± 7.1e-4 \\
IC & CIFAR-100 10-shot & MiX/B/16 & 65 & 248 & 8.77e-2 ± 1.9e-3 & 8.77e-2 ± 1.9e-3 & 2.71e-2 ± 1.2e-3 & 2.60e-2 ± 1.2e-3 & \bfseries 8.61e-3 ± 9.5e-4 \\
IC & CIFAR-100 10-shot & MiX/L/16 & 67 & 313 & 1.05e-1 ± 3.1e-3 & 1.05e-1 ± 3.1e-3 & 4.85e-2 ± 2.6e-3 & 4.76e-2 ± 1.7e-3 & \bfseries 1.55e-2 ± 1.6e-3 \\
IC & CIFAR-100 10-shot & ViT/B/16 & 67 & 354 & 8.98e-2 ± 2.0e-3 & 8.98e-2 ± 2.0e-3 & 8.98e-2 ± 2.0e-3 & 5.60e-2 ± 1.8e-3 & \bfseries 1.73e-2 ± 1.8e-3 \\
IC & CIFAR-100 10-shot & ViT/S/16 & 67 & 450 & 6.84e-2 ± 1.1e-3 & 2.11e-2 ± 6.6e-4 & 3.35e-2 ± 8.6e-4 & 2.47e-2 ± 7.4e-4 & \bfseries 1.15e-2 ± 7.5e-4 \\
IC & CIFAR-100 25-shot & BiT/101/3 & 41 & 38 & 8.77e-2 ± 5.6e-3 & 8.77e-2 ± 5.6e-3 & 4.44e-2 ± 3.5e-3 & 4.29e-2 ± 3.4e-3 & \bfseries 9.32e-3 ± 3.0e-3 \\
IC & CIFAR-100 25-shot & BiT/50/1 & 55 & 109 & 7.31e-2 ± 2.0e-3 & 2.35e-2 ± 1.5e-3 & 3.65e-2 ± 1.8e-3 & 2.36e-2 ± 1.5e-3 & \bfseries 2.00e-2 ± 1.8e-3 \\
IC & CIFAR-100 25-shot & MiX/B/16 & 64 & 202 & 1.08e-1 ± 2.3e-3 & 4.75e-2 ± 1.6e-3 & 2.10e-2 ± 9.4e-4 & 2.08e-2 ± 9.3e-4 & \bfseries 8.15e-3 ± 1.1e-3 \\
IC & CIFAR-100 25-shot & MiX/L/16 & 62 & 185 & 9.79e-2 ± 2.2e-3 & 9.79e-2 ± 2.2e-3 & 3.67e-2 ± 1.7e-3 & 2.79e-2 ± 1.3e-3 & \bfseries 8.47e-3 ± 1.6e-3 \\
IC & CIFAR-100 25-shot & ViT/B/16 & 66 & 355 & 1.07e-1 ± 1.9e-3 & 1.07e-1 ± 1.9e-3 & 6.54e-2 ± 1.6e-3 & \bfseries 4.81e-2 ± 1.4e-3 & 1.20e-1 ± 1.4e-3 \\
IC & CIFAR-100 25-shot & ViT/S/16 & 66 & 416 & 8.03e-2 ± 1.2e-3 & 2.19e-2 ± 7.4e-4 & 3.13e-2 ± 8.4e-4 & 2.19e-2 ± 7.0e-4 & \bfseries 1.34e-2 ± 8.5e-4 \\
IC & CIFAR-100 5-shot & BiT/101/3 & 47 & 59 & 5.94e-2 ± 3.2e-3 & 5.94e-2 ± 3.2e-3 & 5.94e-2 ± 3.2e-3 & 4.57e-2 ± 2.8e-3 & \bfseries 1.58e-2 ± 2.6e-3 \\
IC & CIFAR-100 5-shot & BiT/50/1 & 57 & 98 & 4.87e-2 ± 1.3e-3 & 4.87e-2 ± 1.3e-3 & \bfseries 1.69e-2 ± 8.8e-4 & 4.91e-2 ± 1.3e-3 & 1.95e-2 ± 1.0e-3 \\
IC & CIFAR-100 5-shot & MiX/B/16 & 66 & 304 & 7.07e-2 ± 1.2e-3 & 7.07e-2 ± 1.2e-3 & 2.78e-2 ± 8.4e-4 & 2.05e-2 ± 7.4e-4 & \bfseries 6.77e-3 ± 6.3e-4 \\
IC & CIFAR-100 5-shot & MiX/L/16 & 67 & 312 & 7.06e-2 ± 1.6e-3 & 7.06e-2 ± 1.6e-3 & 4.17e-2 ± 1.4e-3 & 3.14e-2 ± 1.1e-3 & \bfseries 1.18e-2 ± 1.3e-3 \\
IC & CIFAR-100 5-shot & ViT/B/16 & 67 & 352 & 6.27e-2 ± 1.6e-3 & 6.27e-2 ± 1.6e-3 & 6.27e-2 ± 1.6e-3 & 5.11e-2 ± 1.4e-3 & \bfseries 1.19e-2 ± 1.2e-3 \\
IC & CIFAR-100 5-shot & ViT/S/16 & 70 & 710 & 6.93e-2 ± 1.2e-3 & \bfseries 2.84e-2 ± 8.2e-4 & 3.88e-2 ± 8.0e-4 & 3.09e-2 ± 7.5e-4 & 6.40e-2 ± 7.7e-4 \\
IC & Caltech101 10-shot & BiT/101/3 & 21 & 14 & 3.07e-1 ± 2.0e-2 & 3.07e-1 ± 2.0e-2 & 1.51e-1 ± 1.3e-2 & 3.54e-2 ± 6.3e-3 & \bfseries 6.42e-3 ± 5.8e-3 \\
IC & Caltech101 10-shot & BiT/50/1 & 33 & 16 & 3.29e-1 ± 1.6e-2 & 7.68e-2 ± 5.0e-3 & 1.13e-1 ± 6.0e-3 & 6.31e-2 ± 4.4e-3 & \bfseries 5.37e-3 ± 2.2e-3 \\
IC & Caltech101 10-shot & MiX/B/16 & 14 & 12 & 1.35e-1 ± 1.4e-2 & 1.35e-1 ± 1.4e-2 & 1.35e-1 ± 1.4e-2 & 2.11e-1 ± 1.7e-2 & \bfseries 3.72e-2 ± 9.7e-3 \\
IC & Caltech101 10-shot & MiX/L/16 & 12 & 11 & 1.25e-1 ± 1.3e-2 & 1.25e-1 ± 1.3e-2 & 1.25e-1 ± 1.3e-2 & 1.92e-1 ± 1.6e-2 & \bfseries 3.73e-2 ± 1.5e-2 \\
IC & Caltech101 10-shot & ViT/B/16 & 34 & 33 & 7.76e-2 ± 4.3e-3 & 7.76e-2 ± 4.3e-3 & 3.11e-2 ± 3.0e-3 & 5.54e-2 ± 4.3e-3 & \bfseries 1.67e-2 ± 5.4e-3 \\
IC & Caltech101 10-shot & ViT/S/16 & 43 & 55 & 1.95e-1 ± 6.0e-3 & 3.41e-2 ± 2.9e-3 & \bfseries 2.40e-2 ± 2.0e-3 & 3.95e-2 ± 3.1e-3 & 3.31e-2 ± 5.3e-3 \\
IC & Caltech101 25-shot & BiT/101/3 & 10 & 3 & 1.15e-1 ± 6.5e-3 & 1.15e-1 ± 6.5e-3 & 1.15e-1 ± 6.5e-3 & 5.23e-2 ± 2.7e-3 & \bfseries 1.13e-2 ± 8.0e-3 \\
IC & Caltech101 25-shot & BiT/50/1 & 28 & 16 & 3.60e-1 ± 1.9e-2 & 8.80e-2 ± 5.5e-3 & 1.43e-1 ± 7.6e-3 & 5.95e-2 ± 4.1e-3 & \bfseries 2.13e-3 ± 1.6e-3 \\
IC & Caltech101 25-shot & MiX/B/16 & 13 & 11 & 8.28e-2 ± 1.2e-2 & 8.28e-2 ± 1.2e-2 & 8.28e-2 ± 1.2e-2 & 1.74e-1 ± 1.7e-2 & \bfseries 2.83e-2 ± 1.3e-2 \\
IC & Caltech101 25-shot & MiX/L/16 & 12 & 12 & 9.66e-2 ± 1.0e-2 & 9.66e-2 ± 1.0e-2 & 9.66e-2 ± 1.0e-2 & 1.03e-1 ± 9.5e-3 & \bfseries 1.98e-2 ± 1.3e-2 \\
IC & Caltech101 25-shot & ViT/B/16 & 27 & 28 & 1.03e-1 ± 5.6e-3 & 3.33e-2 ± 2.5e-3 & 4.46e-2 ± 3.6e-3 & 4.24e-2 ± 3.6e-3 & \bfseries 6.37e-3 ± 5.4e-3 \\
IC & Caltech101 25-shot & ViT/S/16 & 41 & 54 & 1.77e-1 ± 5.4e-3 & 3.79e-2 ± 3.1e-3 & 2.80e-2 ± 1.8e-3 & \bfseries 2.35e-2 ± 2.3e-3 & 2.38e-2 ± 4.7e-3 \\
IC & Caltech101 5-shot & BiT/101/3 & 16 & 13 & 2.12e-1 ± 1.2e-2 & 2.12e-1 ± 1.2e-2 & 2.12e-1 ± 1.2e-2 & 8.82e-2 ± 5.0e-3 & \bfseries 3.17e-3 ± 4.3e-3 \\
IC & Caltech101 5-shot & BiT/50/1 & 46 & 54 & 2.34e-1 ± 6.1e-3 & 4.13e-2 ± 2.1e-3 & 1.61e-2 ± 1.3e-3 & 4.49e-2 ± 2.1e-3 & \bfseries 1.33e-2 ± 2.2e-3 \\
IC & Caltech101 5-shot & MiX/B/16 & 24 & 19 & 2.43e-1 ± 1.2e-2 & 2.43e-1 ± 1.2e-2 & 2.35e-1 ± 1.1e-2 & 1.23e-1 ± 6.0e-3 & \bfseries 3.59e-3 ± 1.9e-3 \\
IC & Caltech101 5-shot & MiX/L/16 & 14 & 13 & 1.38e-1 ± 9.7e-3 & 1.38e-1 ± 9.7e-3 & 1.38e-1 ± 9.7e-3 & 3.19e-2 ± 2.6e-3 & \bfseries 3.19e-2 ± 1.1e-2 \\
IC & Caltech101 5-shot & ViT/B/16 & 38 & 41 & 1.10e-1 ± 6.3e-3 & 1.10e-1 ± 6.3e-3 & 6.02e-2 ± 4.7e-3 & 6.59e-2 ± 4.7e-3 & \bfseries 2.33e-2 ± 6.0e-3 \\
IC & Caltech101 5-shot & ViT/S/16 & 49 & 82 & 1.90e-1 ± 4.7e-3 & 3.82e-2 ± 2.6e-3 & 5.04e-2 ± 2.9e-3 & 4.06e-2 ± 2.7e-3 & \bfseries 2.47e-2 ± 3.8e-3 \\
IC & ImageNet 10-shot & BiT/101/3 & 60 & 118 & 1.27e-1 ± 2.0e-3 & 1.27e-1 ± 2.0e-3 & 7.36e-2 ± 1.1e-3 & 2.13e-2 ± 5.8e-4 & \bfseries 5.95e-3 ± 5.5e-4 \\
IC & ImageNet 10-shot & BiT/50/1 & 68 & 262 & 9.54e-2 ± 7.2e-4 & 9.54e-2 ± 7.2e-4 & \bfseries 5.75e-3 ± 2.0e-4 & 1.77e-2 ± 2.7e-4 & 8.93e-3 ± 2.7e-4 \\
IC & ImageNet 10-shot & MiX/B/16 & 69 & 329 & 9.34e-2 ± 7.9e-4 & 9.34e-2 ± 7.9e-4 & 3.37e-2 ± 2.9e-4 & 1.80e-2 ± 2.7e-4 & \bfseries 5.88e-3 ± 2.5e-4 \\
IC & ImageNet 10-shot & MiX/L/16 & 66 & 249 & 9.83e-2 ± 1.3e-3 & 9.83e-2 ± 1.3e-3 & 9.83e-2 ± 1.3e-3 & 9.48e-3 ± 2.4e-4 & \bfseries 3.81e-3 ± 2.9e-4 \\
IC & ImageNet 10-shot & ViT/B/16 & 67 & 289 & 4.62e-2 ± 7.1e-4 & 4.62e-2 ± 7.1e-4 & 4.62e-2 ± 7.1e-4 & 3.43e-2 ± 4.4e-4 & \bfseries 2.85e-3 ± 2.7e-4 \\
IC & ImageNet 10-shot & ViT/S/16 & 65 & 310 & 4.74e-2 ± 5.6e-4 & 4.74e-2 ± 5.6e-4 & 1.66e-2 ± 2.5e-4 & 1.14e-2 ± 2.4e-4 & \bfseries 1.97e-3 ± 1.4e-4 \\
IC & ImageNet 25-shot & BiT/101/3 & 57 & 100 & 1.42e-1 ± 2.3e-3 & 1.42e-1 ± 2.3e-3 & 6.67e-2 ± 9.1e-4 & 2.18e-2 ± 7.0e-4 & \bfseries 4.86e-3 ± 6.2e-4 \\
IC & ImageNet 25-shot & BiT/50/1 & 68 & 263 & 1.17e-1 ± 9.2e-4 & 1.17e-1 ± 9.2e-4 & \bfseries 4.06e-3 ± 1.7e-4 & 1.70e-2 ± 2.5e-4 & 8.14e-3 ± 2.4e-4 \\
IC & ImageNet 25-shot & MiX/B/16 & 68 & 284 & 9.59e-2 ± 9.3e-4 & 9.59e-2 ± 9.3e-4 & 5.39e-2 ± 4.9e-4 & 1.47e-2 ± 2.7e-4 & \bfseries 2.86e-3 ± 2.3e-4 \\
IC & ImageNet 25-shot & MiX/L/16 & 66 & 226 & 1.03e-1 ± 1.3e-3 & 1.03e-1 ± 1.3e-3 & 1.03e-1 ± 1.3e-3 & 6.09e-3 ± 2.5e-4 & \bfseries 1.94e-3 ± 2.6e-4 \\
IC & ImageNet 25-shot & ViT/B/16 & 67 & 289 & 5.17e-2 ± 8.8e-4 & 5.17e-2 ± 8.8e-4 & 5.17e-2 ± 8.8e-4 & 3.26e-2 ± 5.4e-4 & \bfseries 6.91e-3 ± 4.3e-4 \\
IC & ImageNet 25-shot & ViT/S/16 & 65 & 311 & 5.52e-2 ± 4.4e-4 & 4.12e-2 ± 3.4e-4 & 9.65e-3 ± 2.3e-4 & 1.16e-2 ± 2.2e-4 & \bfseries 3.09e-3 ± 2.4e-4 \\
IC & ImageNet 5-shot & BiT/101/3 & 60 & 124 & 9.24e-2 ± 1.4e-3 & 9.24e-2 ± 1.4e-3 & 9.24e-2 ± 1.4e-3 & 1.01e-2 ± 5.3e-4 & \bfseries 2.55e-3 ± 5.0e-4 \\
IC & ImageNet 5-shot & BiT/50/1 & 69 & 305 & 8.95e-2 ± 6.7e-4 & 8.95e-2 ± 6.7e-4 & 1.53e-2 ± 2.2e-4 & 1.03e-2 ± 2.3e-4 & \bfseries 4.00e-3 ± 2.1e-4 \\
IC & ImageNet 5-shot & MiX/B/16 & 70 & 394 & 9.09e-2 ± 7.2e-4 & 9.09e-2 ± 7.2e-4 & 3.01e-2 ± 2.8e-4 & 1.45e-2 ± 2.5e-4 & \bfseries 3.57e-3 ± 2.3e-4 \\
IC & ImageNet 5-shot & MiX/L/16 & 67 & 240 & 7.99e-2 ± 9.7e-4 & 7.99e-2 ± 9.7e-4 & 7.99e-2 ± 9.7e-4 & 5.66e-3 ± 3.1e-4 & \bfseries 1.63e-3 ± 2.4e-4 \\
IC & ImageNet 5-shot & ViT/B/16 & 68 & 361 & 4.11e-2 ± 6.3e-4 & 4.11e-2 ± 6.3e-4 & 4.11e-2 ± 6.3e-4 & 2.88e-2 ± 3.6e-4 & \bfseries 4.97e-3 ± 2.7e-4 \\
IC & ImageNet 5-shot & ViT/S/16 & 66 & 323 & 4.20e-2 ± 4.1e-4 & 4.20e-2 ± 4.1e-4 & 2.40e-2 ± 2.6e-4 & 1.44e-2 ± 2.2e-4 & \bfseries 3.00e-3 ± 1.7e-4 \\
\end{tabular}
    \caption{
    Extrapolation Results for Vision Tasks. See Section \ref{section:scaling_benchmark__vision} for more details. Numbers for M1, M2, M3, and M4 obtained via correspondence with authors of \cite{Alabdulmohsi2022revisiting}. 
    }
    \label{table:scaling_laws_benchmark_dataset__Vision}
\end{table}
\FloatBarrier

\subsection{Language}
\label{section:scaling_benchmark__language}
Using the scaling laws benchmark of \cite{Alabdulmohsi2022revisiting}, we evaluate how well various functional forms extrapolate performance on language tasks as training dataset size increases. In this language subset of the benchmark, the tasks that are evaluated are error rate on each of various downstream tasks from the BIG-Bench (BB) \cite{srivastava2022beyond} benchmark and upstream test cross-entropy of various models trained to do language modeling (LM) and neural machine translation (NMT). All LM and BB tasks use a decoder-only language model. As can be seen in Table  \ref{table:scaling_laws_benchmark_dataset__language}, BNSL (TODO: make sure BNSL abbreviation is defined somewhere) yields extrapolations with the lowest RMSLE for the largest number of tasks of any of functional forms. 

TODO: Should these sentence be removed.
The one task subset where the extrapolations of BNSL are comparable (rather than significantly better) is upstream cross entropy of language modeling because in that task the RMSLE is already very low (i.e. lower than 1e-3) such that there is not much headroom to improve further. Sentence about 

To view all plots of the BNSL on each of these tasks, see Figures
\ref{fig:scaling_laws_benchmark_dataset__big_bench},
\ref{fig:scaling_laws_benchmark_dataset__nmt},
\ref{fig:scaling_laws_benchmark_dataset__language_modeling} in Appendix \ref{section:Plots_of_BNSL_Extrapolations}.

To view plots of M1, M2, M3, and M4 on these tasks, see Figure 8 of \cite{Alabdulmohsi2022revisiting}.


\FloatBarrier
\begin{table}[htbp]

\tiny
\setlength\tabcolsep{3.1pt} 
\begin{tabular}
%{p{.02\textwidth}p{.165\textwidth}p{.095\textwidth}p{.01\textwidth}p{.01\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}}
{p{.021\textwidth}p{.165\textwidth}p{.111\textwidth}p{.028\textwidth}p{.025\textwidth}p{.11\textwidth}p{.11\textwidth}p{.11\textwidth}p{.11\textwidth}p{.11\textwidth}}
%\begin{tabular}{llllrrrrrrrrrrrrl}
Domain & \hspace{.9cm}Task & Model & Train Points & Test Points & M1 $\downarrow$ & M2 $\downarrow$ & M3 $\downarrow$ & M4 $\downarrow$ & BNSL $\downarrow$ \\
\hline
BB & date understanding, 1-shot & 2.62e+8 Param & 19 & 24 & 3.19e-2 ± 9.6e-4 & 3.09e-2 ± 9.2e-4 & \highlight{4.67e-3 ± 1.4e-4} & 1.49e-2 ± 5.9e-4 & 4.96e-3 ± 4.8e-5 \\
BB & date understanding, 2-shot & 2.62e+8 Param & 19 & 24 & 2.86e-2 ± 6.2e-4 & 2.44e-2 ± 5.6e-4 & 4.83e-3 ± 4.1e-4 & 1.58e-2 ± 5.0e-4 & \highlight{2.55e-3 ± 6.2e-4} \\
BB & linguistic mappings, 1-shot & 2.62e+8 Param & 19 & 24 & 1.66e-2 ± 5.5e-4 & \highlight{1.41e-2 ± 4.7e-4} & 1.66e-2 ± 5.5e-4 & 1.57e-2 ± 4.8e-4 & 2.22e-2 ± 8.2e-4 \\
BB & linguistic mappings, 2-shot & 2.62e+8 Param & 19 & 24 & 1.70e-2 ± 6.5e-4 & 1.30e-2 ± 5.4e-4 & 1.70e-2 ± 6.5e-4 & 9.25e-3 ± 5.1e-4 & \highlight{8.09e-3 ± 5.1e-4} \\
BB & mult data wrangling, 1-shot & 2.62e+8 Param & 19 & 24 & 1.07e-2 ± 1.0e-3 & 6.71e-3 ± 7.6e-4 & 1.07e-2 ± 1.0e-3 & 8.27e-3 ± 8.4e-4 & \highlight{6.17e-3 ± 8.4e-4} \\
BB & mult data wrangling, 2-shot & 2.62e+8 Param & 19 & 24 & 1.57e-2 ± 1.5e-3 & 7.22e-3 ± 8.9e-4 & 1.57e-2 ± 1.5e-3 & \highlight{5.01e-3 ± 5.0e-4} & 5.45e-3 ± 9.2e-4 \\
BB & qa wikidata, 1-shot & 2.62e+8 Param & 19 & 24 & \highlight{4.27e-3 ± 8.9e-4} & 5.14e-3 ± 5.3e-4 & 4.27e-3 ± 8.9e-4 & 5.05e-3 ± 5.6e-4 & 4.34e-3 ± 6.1e-4 \\
BB & qa wikidata, 2-shot & 2.62e+8 Param & 19 & 24 & 4.39e-3 ± 7.0e-4 & 7.35e-3 ± 6.1e-4 & 4.39e-3 ± 7.0e-4 & 7.12e-3 ± 6.0e-4 & \highlight{4.20e-3 ± 6.0e-4} \\
BB & unit conversion, 1-shot & 2.62e+8 Param & 19 & 24 & 8.30e-3 ± 4.4e-4 & 6.77e-3 ± 4.0e-4 & \highlight{1.48e-3 ± 2.7e-4} & 2.32e-3 ± 2.3e-4 & 6.32e-3 ± 2.5e-4 \\
BB & unit conversion, 2-shot & 2.62e+8 Param & 19 & 24 & 1.07e-2 ± 4.4e-4 & 9.15e-3 ± 4.7e-4 & 7.50e-3 ± 5.5e-4 & \highlight{2.83e-3 ± 4.8e-4} & 5.21e-3 ± 5.2e-4 \\
LM & upstream test cross-entropy& 1.07e+9 Param & 44 & 40 & 1.71e-2 ± 6.0e-4 & 1.02e-3 ± 3.5e-5 & 4.50e-3 ± 5.9e-5 & \highlight{3.79e-4 ± 4.0e-5} & 8.26e-4 ± 3.2e-5 \\
LM & upstream test cross-entropy& 4.53e+8 Param & 44 & 40 & 1.65e-2 ± 6.6e-4 & 6.47e-4 ± 8.5e-5 & 6.58e-4 ± 6.6e-5 & 8.54e-4 ± 4.7e-5 & \highlight{5.10e-4 ± 7.7e-5} \\
LM & upstream test cross-entropy& 2.62e+8 Param & 156 & 20 & 1.55e-2 ± 7.2e-4 & 1.01e-3 ± 9.4e-5 & 3.97e-3 ± 1.3e-4 & \highlight{9.37e-4 ± 9.7e-5} & 1.80e-3 ± 5.6e-5 \\
LM & upstream test cross-entropy& 1.34e+8 Param & 48 & 48 & 1.43e-2 ± 4.8e-4 & 1.33e-3 ± 6.5e-5 & \highlight{6.46e-4 ± 5.1e-5} & 8.14e-4 ± 5.3e-5 & 8.09e-4 ± 5.5e-5 \\
LM & upstream test cross-entropy& 1.68e+7 Param & 236 & 240 & 6.37e-3 ± 9.4e-5 & \highlight{3.08e-4 ± 1.3e-5} & 1.24e-3 ± 3.2e-5 & 3.27e-4 ± 1.5e-5 & 4.05e-4 ± 1.8e-5 \\
NMT & upstream test cross-entropy & 28 Enc, 6 Dec & 9 & 1 & 1.71e-1 ± 0 & 5.63e-2 ± 0 & 3.37e-2 ± 0 & 1.50e-2 ± 0 & \highlight{5.13e-3 ± 0} \\
NMT & upstream test cross-entropy & 6 Enc, 28 Dec & 10 & 1 & 2.34e-1 ± 0 & 5.27e-2 ± 0 & 1.65e-2 ± 0 & 3.21e-2 ± 0 & \highlight{9.81e-3 ± 0} \\
NMT & upstream test cross-entropy & 6 Enc, 6 Dec & 10 & 1 & 2.62e-1 ± 0 & 3.84e-2 ± 0 & 8.92e-2 ± 0 & \highlight{1.05e-2 ± 0} & 1.41e-2 ± 0 \\
NMT & upstream test cross-entropy & Dec-only, LM & 10 & 1 & 2.52e-1 ± 0 & 1.03e-2 ± 0 & 3.28e-2 ± 0 & 8.88e-3 ± 0 & \highlight{2.79e-3 ± 0} \\
NMT & upstream test cross-entropy & Trans-E, LSTM-D & 9 & 1 & 1.90e-1 ± 0 & 1.26e-2 ± 0 & 6.32e-2 ± 0 & 1.31e-2 ± 0 & \highlight{3.08e-3 ± 0} \\    
\end{tabular}
    \caption{
    Extrapolation Results for Language Tasks. See Section \ref{section:scaling_benchmark__language} for more details. Numbers for M1, M2, M3, and M4 obtained via correspondence with authors of \cite{Alabdulmohsi2022revisiting}.
    }
    \label{table:scaling_laws_benchmark_dataset__language}
\end{table}
\FloatBarrier


\FloatBarrier
\begin{table}[htbp]

\tiny
\setlength\tabcolsep{3.1pt} 
\begin{tabular}
%{p{.02\textwidth}p{.165\textwidth}p{.095\textwidth}p{.01\textwidth}p{.01\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}}
{p{.021\textwidth}p{.165\textwidth}p{.111\textwidth}p{.028\textwidth}p{.022\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}p{.099\textwidth}}
%\begin{tabular}{llllrrrrrrrrrrrrl}
Domain & \hspace{.9cm}Task & Model & Train Points & Test Points & M1 $\downarrow$ & M2 $\downarrow$ & M3 $\downarrow$ & M4 $\downarrow$ & BNSL $\downarrow$ \\
\hline
BB & date understanding, 1-shot & 2.62e+8 Param & 19 & 24 & 3.19e-2 ± 9.6e-4 & 3.09e-2 ± 9.2e-4 & \bfseries 4.67e-3 ± 1.4e-4 & 1.49e-2 ± 5.9e-4 & 4.96e-3 ± 4.8e-5 \\
BB & date understanding, 2-shot & 2.62e+8 Param & 19 & 24 & 2.86e-2 ± 6.2e-4 & 2.44e-2 ± 5.6e-4 & 4.83e-3 ± 4.1e-4 & 1.58e-2 ± 5.0e-4 & \bfseries 2.55e-3 ± 6.2e-4 \\
BB & linguistic mappings, 1-shot & 2.62e+8 Param & 19 & 24 & 1.66e-2 ± 5.5e-4 & \bfseries 1.41e-2 ± 4.7e-4 & 1.66e-2 ± 5.5e-4 & 1.57e-2 ± 4.8e-4 & 2.22e-2 ± 8.2e-4 \\
BB & linguistic mappings, 2-shot & 2.62e+8 Param & 19 & 24 & 1.70e-2 ± 6.5e-4 & 1.30e-2 ± 5.4e-4 & 1.70e-2 ± 6.5e-4 & 9.25e-3 ± 5.1e-4 & \bfseries 8.09e-3 ± 5.1e-4 \\
BB & mult data wrangling, 1-shot & 2.62e+8 Param & 19 & 24 & 1.07e-2 ± 1.0e-3 & 6.71e-3 ± 7.6e-4 & 1.07e-2 ± 1.0e-3 & 8.27e-3 ± 8.4e-4 & \bfseries 6.17e-3 ± 8.4e-4 \\
BB & mult data wrangling, 2-shot & 2.62e+8 Param & 19 & 24 & 1.57e-2 ± 1.5e-3 & 7.22e-3 ± 8.9e-4 & 1.57e-2 ± 1.5e-3 & \bfseries 5.01e-3 ± 5.0e-4 & 5.45e-3 ± 9.2e-4 \\
BB & qa wikidata, 1-shot & 2.62e+8 Param & 19 & 24 & \bfseries 4.27e-3 ± 8.9e-4 & 5.14e-3 ± 5.3e-4 & 4.27e-3 ± 8.9e-4 & 5.05e-3 ± 5.6e-4 & 4.34e-3 ± 6.1e-4 \\
BB & qa wikidata, 2-shot & 2.62e+8 Param & 19 & 24 & 4.39e-3 ± 7.0e-4 & 7.35e-3 ± 6.1e-4 & 4.39e-3 ± 7.0e-4 & 7.12e-3 ± 6.0e-4 & \bfseries 4.20e-3 ± 6.0e-4 \\
BB & unit conversion, 1-shot & 2.62e+8 Param & 19 & 24 & 8.30e-3 ± 4.4e-4 & 6.77e-3 ± 4.0e-4 & \bfseries 1.48e-3 ± 2.7e-4 & 2.32e-3 ± 2.3e-4 & 6.32e-3 ± 2.5e-4 \\
BB & unit conversion, 2-shot & 2.62e+8 Param & 19 & 24 & 1.07e-2 ± 4.4e-4 & 9.15e-3 ± 4.7e-4 & 7.50e-3 ± 5.5e-4 & \bfseries 2.83e-3 ± 4.8e-4 & 5.21e-3 ± 5.2e-4 \\
LM & upstream test cross-entropy& 1.07e+9 Param & 44 & 40 & 1.71e-2 ± 6.0e-4 & 1.02e-3 ± 3.5e-5 & 4.50e-3 ± 5.9e-5 & \bfseries 3.79e-4 ± 4.0e-5 & 8.26e-4 ± 3.2e-5 \\
LM & upstream test cross-entropy& 4.53e+8 Param & 44 & 40 & 1.65e-2 ± 6.6e-4 & 6.47e-4 ± 8.5e-5 & 6.58e-4 ± 6.6e-5 & 8.54e-4 ± 4.7e-5 & \bfseries 5.10e-4 ± 7.7e-5 \\
LM & upstream test cross-entropy& 2.62e+8 Param & 156 & 20 & 1.55e-2 ± 7.2e-4 & 1.01e-3 ± 9.4e-5 & 3.97e-3 ± 1.3e-4 & \bfseries 9.37e-4 ± 9.7e-5 & 1.80e-3 ± 5.6e-5 \\
LM & upstream test cross-entropy& 1.34e+8 Param & 48 & 48 & 1.43e-2 ± 4.8e-4 & 1.33e-3 ± 6.5e-5 & \bfseries 6.46e-4 ± 5.1e-5 & 8.14e-4 ± 5.3e-5 & 8.09e-4 ± 5.5e-5 \\
LM & upstream test cross-entropy& 1.68e+7 Param & 236 & 240 & 6.37e-3 ± 9.4e-5 & \bfseries 3.08e-4 ± 1.3e-5 & 1.24e-3 ± 3.2e-5 & 3.27e-4 ± 1.5e-5 & 4.05e-4 ± 1.8e-5 \\
NMT & upstream test cross-entropy & 28 Enc, 6 Dec & 9 & 1 & 1.71e-1 ± 0 & 5.63e-2 ± 0 & 3.37e-2 ± 0 & 1.50e-2 ± 0 & \bfseries 5.13e-3 ± 0 \\
NMT & upstream test cross-entropy & 6 Enc, 28 Dec & 10 & 1 & 2.34e-1 ± 0 & 5.27e-2 ± 0 & 1.65e-2 ± 0 & 3.21e-2 ± 0 & \bfseries 9.81e-3 ± 0 \\
NMT & upstream test cross-entropy & 6 Enc, 6 Dec & 10 & 1 & 2.62e-1 ± 0 & 3.84e-2 ± 0 & 8.92e-2 ± 0 & \bfseries 1.05e-2 ± 0 & 1.41e-2 ± 0 \\
NMT & upstream test cross-entropy & Dec-only, LM & 10 & 1 & 2.52e-1 ± 0 & 1.03e-2 ± 0 & 3.28e-2 ± 0 & 8.88e-3 ± 0 & \bfseries 2.79e-3 ± 0 \\
NMT & upstream test cross-entropy & Trans-E, LSTM-D & 9 & 1 & 1.90e-1 ± 0 & 1.26e-2 ± 0 & 6.32e-2 ± 0 & 1.31e-2 ± 0 & \bfseries 3.08e-3 ± 0 \\
\end{tabular}
    \caption{
    Extrapolation Results for Language Tasks. See Section \ref{section:scaling_benchmark__language} for more details. Numbers for M1, M2, M3, and M4 obtained via correspondence with authors of \cite{Alabdulmohsi2022revisiting}.
    }
    \label{table:scaling_laws_benchmark_dataset__language}
\end{table}
\FloatBarrier

%LM & upstream test cross-entropy& 1.07e+9 Param & 44 & 40 & 1.71e-2 ± 6.0e-4 & 1.02e-3 ± 3.5e-5 & 4.50e-3 ± 5.9e-5 & \bfseries 3.79e-4 ± 4.0e-5 & \bfseries 8.26e-4 ± 3.2e-5 \\
%LM & upstream test cross-entropy& 1.34e+8 Param & 48 & 48 & 1.43e-2 ± 4.8e-4 & 1.33e-3 ± 6.5e-5 & \bfseries 6.46e-4 ± 5.1e-5 & \bfseries 8.14e-4 ± 5.3e-5 & \bfseries 8.09e-4 ± 5.5e-5 \\
%LM & upstream test cross-entropy& 1.68e+7 Param & 236 & 240 & 6.37e-3 ± 9.4e-5 & \bfseries 3.08e-4 ± 1.3e-5 & 1.24e-3 ± 3.2e-5 & \bfseries 3.27e-4 ± 1.5e-5 & \bfseries 4.05e-4 ± 1.8e-5 \\
%LM & upstream test cross-entropy& 2.62e+8 Param & 156 & 20 & 1.55e-2 ± 7.2e-4 & 1.01e-3 ± 9.4e-5 & 3.97e-3 ± 1.3e-4 & \bfseries 9.37e-4 ± 9.7e-5 & 1.80e-3 ± 5.6e-5 \\
%LM & upstream test cross-entropy& 4.53e+8 Param & 44 & 40 & 1.65e-2 ± 6.6e-4 & \bfseries 6.47e-4 ± 8.5e-5 & \bfseries 6.58e-4 ± 6.6e-5 & \bfseries 8.54e-4 ± 4.7e-5 & \bfseries 5.10e-4 ± 7.7e-5 \\
%\end{tabular}
%    \caption{
%    Extrapolation Results for Language Tasks. See Section \ref{section:scaling_benchmark__language} for more details. Numbers for M1, M2, M3, and M4 obtained via correspondence with authors of \cite{Alabdulmohsi2022revisiting}. Bolded if lowest in row or below 1e-3.
%    }
%    \label{table:scaling_laws_benchmark_dataset__language}
%\end{table}

\subsection{Non-Monotonic Scaling}
We show that BNSL accurately models non-monotonic scaling behaviors present in double descent \citep{nakkiran2021deep} in Figure \ref{fig:double_descent}. Other functional forms are mathematically incapable of expressing non-monotonic behaviours (as shown in Section 3).

\FloatBarrier
\begin{figure*}[htbp]
    \centering


\includegraphics[width=0.48\textwidth]{figures/double_descent/double_descent__model_size.png}
\includegraphics[width=0.48\textwidth]{figures/double_descent/double_descent__dataset_size_1.png}

    \caption{
    Fit of BNSL to Double Descent. Both plots are of transformers trained to do neural machine translation via minimizing cross-entropy. Experimental data of left figure is obtained from Figure 8 top of \cite{nakkiran2021deep}; ``Model Width" on the x-axis refers to embedding dimension $d_{model}$ of the transformer. Experimental data of right figure is obtained from Figure 11b of \cite{nakkiran2021deep}.
    }
    \label{fig:double_descent}
\end{figure*}
\FloatBarrier

\subsection{Inflection Points}
\label{section:Inflection_Points}
We show that BNSL is capable of modeling and extrapolating the scaling behavior of tasks that have an inflection point on a linear-linear plot such as the task of arithmetic (4 digit addition). Other functional forms are mathematically incapable of expressing inflection points on a linear-linear plot (as shown in Section 3) and as a result are mathematically incapable of expressing and modeling inflection points (on a linear-linear plot) that are present in the scaling behaviour of 4 digit addition. In Figure \ref{fig:arithmetic} left, we show that BNSL expresses and accurately models the inflection point present in the scaling behaviour of 4 digit addition and as a result accurately extrapolates the scaling behaviour of 4 digit addition.

\FloatBarrier
\begin{figure*}[htbp]
    \centering


%\includegraphics[width=0.48\textwidth]{figures/arithmetic/4_digit_addition__dataset_size.png}
\includegraphics[width=0.48\textwidth]{figures/arithmetic/4_digit_addition__dataset_size__very_first_version.png}
\includegraphics[width=0.48\textwidth]{figures/arithmetic/4_digit_addition__dataset_size__very_first_version__simulation_limit.png}

    \caption{
    4 Digit Addition. Note that these plots are linear-linear. Each point in the left plot is the mean of greater than 100 seeds at that dataset size. In the left plot, each point is gathered from a model trained to do the task of 4 digit addition. In the right plot, each point is gathered from a noiseless simulation of the BNSL of the task of 4 digit addition.
    }
    \label{fig:arithmetic}
\end{figure*}
\FloatBarrier

\subsection{The Limit of the Predictability of Scaling Behavior}
\label{section:limit_of_agi_superforecasting}
We use BNSL to glean insights about the limit of the predictability of scaling behavior. Recent papers \citep{ganguli2022predictability, wei2022emergent} have advertised many task as having ``unpredictable" scaling behavior, the most famous of which being the task of arithmetic. In the previous section and in Figure \ref{fig:arithmetic} left, we successfully predicted (i.e. extrapolated) the scaling behavior of 4 digit addition (arithmetic). However, we are only able to accurately extrapolate the scaling behaviour if given some points from training runs with a training dataset size of at least 720, and the break in which the scaling behaviour of 4 digit addition transitions from one power law to another steeper power law happens at around training dataset size of 415. Ideally, one would like be able to extrapolate the entire scaling behavior by fitting only points from before the break. In Figure \ref{fig:arithmetic} right, we use a noiseless simulation of the BNSL of 4 digit addition to show what would happen if one had infinitely many training runs / seeds to average out all the noisy deviation between runs such that one could recover (i.e. learn via a curve-fitting library such as SciPy \cite{virtanen2020scipy}) the learned constant of the BNSL as well as possible. When using this noiseless simulation, we find that we are only able to accurately extrapolate the scaling behaviour if given some points from training runs with a training dataset size of at least 415, which is very close to the break. This implies that very near to the break there is limit as to how small the supremum of the x-axis of the points used for fitting can be if one wants to perfectly extrapolate the scaling behavior, even if one has infinitely many seeds / training runs.

\subsection{Reinforcement Learning}

TODO: Does RL just go in the appendix because we don't have enough points to get good extrapolations for RL?

\FloatBarrier
\begin{figure*}[htbp]
    \centering


\includegraphics[width=0.48\textwidth]{figures/rl/reanalyze/reanalyze__ms_pacman_dataset_size__fit.png}


    \caption{
    Fit of BNSL to Figure 1 of \cite{schrittwieser2021online}.
    }
    \label{fig:rl_scaling}
\end{figure*}
\FloatBarrier

%\subsection{BIG Bench Emergent}
%Probably will just finish it for rebuttals

==> old__not_used_anymore/sections_ir/sec_intro.tex <==

\section{Introduction}
The number of model parameters, amount of compute used for training, and training dataset size of the most capable artificial neural networks keeps increasing and will probably keep rapidly increasing for the foreseeable future. However, no organization currently has direct access to these larger resources of the future; and it has been empirically verified many, many times (e.g., see Figure 2 (right) of \cite{tolstikhin2021mlp}) that methods which perform best at smaller scales often are no longer the best performing methods at larger scales. To work on, identify, and steer the methods that are most probable to stand the test-of-time as these larger resources come online, one needs a way to predict how all relevant performance evaluation metrics of artificial neural networks vary in all relevant settings as scale increases. 


\todo[inline]{don't copy the abstract (exactly), paraphrase}
To address this need, we present a smoothly broken power law functional form, referred to by us as a \textbf{broken neural scaling law (BNSL)}, that accurately models the scaling behaviors of artificial neural networks for each task from a very large and diverse set of upstream and downstream (i.e. zero-shot, prompted, and fine-tuned) tasks. These tasks include large-scale vision tasks, large-scale unsupervised language tasks, arithmetic, and reinforcement learning. This functional form yields extrapolations of scaling behavior that often are an order of magnitude more accurate than previous functional forms for modeling the scaling behavior of artificial neural networks. Moreover, this functional form accurately models the non-monotonic transitions present in the scaling behavior of phenomena such as double descent and the delayed, sharp transitions present in the scaling behavior of tasks such as arithmetic.


%One collects some experimental data in the smaller (compute, data, or number of parameters) regime, and then fits a neural scaling law functional form (e.g. via a curve fitting library such as SciPy \cite{virtanen2020scipy}.

%Currently variants of power laws branded as neural scaling laws are main means one uses to make such predictions. One collects some experimental data in the smaller (compute, data, or number of parameters) regime, and then fits a neural scaling law functional form (e.g. via a curve fitting library such as SciPy \cite{virtanen2020scipy}.

%Neural Scaling Laws as they currently are used have some issues. (TODO: this is tricky to phrase because scaling laws for transfer exists and is equivalent to ours)

\iffalse

\section{DK Introduction}
\label{sec:intro}

\todo[inline]{TODO: this needs references all over the place}


%Conventional wisdom and machine learning has long held that more data is always better, but there is a sweet spot for the number of parameters or amount of training: too much of either risks overfitting.
%For modern deep learning, however it seems that more is (almost) always better. % TODO: reference other results like double descent?  Or probably that should come later...
In the largest scale regimes of modern deep learning, it seems that increasing the number of model parameters, amount of compute used for training, or training dataset size (almost) always yields better results. % TODO: reference other results like double descent?  Or probably that should come later...
In fact, scaling up deep learning seems to yield predictable performance improvements, which can be modeled using neural scaling laws.
Remarkably, the same simple functional form, a modified power law, applies equally well to data, parameters, and compute, the three axes along which scaling is measured.
%, provided that none of the three is a bottleneck (TODO: more details on that?). Ethan: It works fine even if bottlenecked.

Currently, the main practical value of neural scaling laws is in forecasting the performance of larger models and datasets without needing to train or collect them.  
Indeed, several works have shown that models that underperform at smaller scales can be predicted to reach state of the art performance at larger scales \citep{}, although such predictions have not always held up \citep{}.
However, it is difficult to translate predictions about performance metrics such as negative log likelihood into predictions about qualitative behaviors and capabilities.
For instance, \citet{GPT} famously document the emergence of in-context meta-learning in large-scale language models.
``Downstream'' performance, i.e.\ that which is measured on metrics other than the training loss, reveals striking discontinuities as a function of scale. % TODO: note that it's not all downstream, and discuss fine-tuning vs. 0-shot
Models suddenly go from near-chance level to state-of-the-art performance on tasks such as TODO once a critical scale is reached.

%TODO: say something more here about how we crush it 

Predicting the emergence of novel capabilities at scale could prove crucial to responsibly developing and deploying increasingly advanced AI systems. % TODO: say more, e.g. mention deception or something?
Doing so requires methods of identifying and measuring relevant capabilities, and scaling laws that can accurately forecast how these capabilities develop at scale. % of modelling their learning dynamics.
However, the functional forms of scaling laws applied in prior work are not up to this challenge.

One salient defect is that they can only represent monotonic functions.
They thus fail to model the striking phenomena of double-descent \citep{}, where increased scale temporarily decreases test performance before ultimately leading to further improvements. %, and grokking \citep{}, where test performance remains near chance levels 
They also lack the expressive power to model inflection points, which can be observed empirically for many downstream tasks, and even some upstream tasks, such as our $N$-digit arithmetic task, or the modular arithmetic task introduced by \citet{grokking} in their work on ``grokking''. 
%For this task, test performance remains near chance levels long after training accuracy has reached 100\% before eventually climbing towards 100\% as well on synthetic arithmetic tasks.
%, and grokking \citep{}, where test performance remains near chance levels long after training accuracy has reached 100\% before eventually climbing towards 100\% as well on synthetic arithmetic tasks.
%Such discontinuities can sometimes even be observed on the ``upstream'' test loss; for instance, we observe them in a simple $N$-digit arithmetic task.
%Another striking phenomena of modern deep learning that 

%also fail to fit the striking phenomena of double-descent \citep{}, where increased scale temporarily decreases test performance before ultimately leading to further improvements.%, and grokking \citep{}, where test performance remains near chance levels long after training accuracy has reached 100\% before eventually climbing towards 100\% as well on synthetic arithmetic tasks.
%Modelling, predicting, and ultimately understanding these phenomena will 
Our work presents a functional form capable of modeling all of these diverse behaviors, and empirically validates it's effectiveness in extrapolating scaling behavior.
%Besides the qualitative di
%TODO: last 2 sentences above are now a bit out of place...
TODO: say something more here about how we crush it (i.e. enumerate all the scaling data we fit).

\fi

%TODO:  Say something like: "Sometimes the non-broken Scaling laws don't even work upstream when you have weird stuff like Grokking or double descent or unusual data sets like our N-digit addition".




\iffalse
\subsection{old Introduction}


%\textbf{\texttt{http://icml.cc/}}
\todo[inline]{motivation: why scaling laws?}
%Machine learning involves optimizing an upstream training objective and evaluating downstream metric(s).

%The endgame of machine learning is going to involve training models with more parameters than the human brain on the entire internet. To make claims today about what machine learning methods will be most effective during the endgame, we must rely on forecasts because no organization currently has enough compute to run these future workloads empirically. The measurement that makes the most sense to forecast is downstream task performance scaling because TODO

One of the principal goals of deep learning research is to find a functional form that characterizes the relationship between performance and scale in all settings. Such a functional form would allow one to better predict that which scales best on all the evaluations that one cares about. TODO: Revisiting NSL had pretty good list of why to care about scaling laws. In pursuit of this goal, we present some key results.

%In this paper, we focus on the 190 downstream task scaling evaluations reported in the GPT-3 arXiv paper because it reports the downstream scaling information for the largest number of tasks of any paper we are aware of.

%main result:
\ir{We demonstrate that the following functional form (also known as smoothly broken power law) is accurately capturing (and extrapolating) multiple performance metrics on a wide range of downstream tasks, in several settings
$
y =  a + \left(\frac{b}{x}\right)^c \prod_{i=1}^n \left(1 + \left(\frac{x}{d_i}\right)^{f_i}\right)^{-g_i}.
$
}

%----IR
%The endgame of machine learning is going to involve training models with more parameters than the human brain on the entire internet. To make claims today about what machine learning methods will be most effective during the endgame, we must rely on forecasts because no organization currently has enough compute to run these future workloads empirically. The measurement that makes the most sense to forecast is downstream task performance scaling because TODO

%One of the principal goals of deep learning research is to find a single functional form that characterizes the relationship between performance and scale in all settings. In pursuit of this goal, we present some key results.  %% IR: a bit controversial statement about finding a single functional form as one of the principal goals of DL.

%In this paper, we focus on the 190 downstream task scaling evaluations reported in the GPT-3 arXiv paper because it reports the downstream scaling information for the largest number of tasks of any paper we are aware of.
%----
\fi

==> old__not_used_anymore/sections_ir/sec_related.tex <==
\section{Related Work}
To the best of our knowledge,\citet{cortes1994learning} was the first paper to model the scaling of multilayer neural network's performance as a power law 
%(also known as a scaling law) (plus a constant) \ir{[I would delete both those phrases in ()] } 
of the form $y=ax^b + c$ in which $x$ refers to training dataset size and $y$ refers to test error.
Later, \citet{2017arXiv171200409H} showed that this functional form holds over many orders of magnitude, while \citet{DBLP:journals/corr/abs-1909-12673} demonstrated  that the same functional form applies when $x$ refers to model size (number of parameters). \citet{icm2020arXiv200108361K} brought ``neural" scaling laws to the mainstream and showed that there is an additional scaling law with respect to compute. \citet{DBLP:journals/corr/abs-2106-04560} introduced the functional form $y=a(x+d)^b + c$, where  d represents the scale at which the performance starts to improve beyond the  random guess loss (a constant) and transitions to a  power law scaling regime. \citet{abnar2021exploring} proposed a functional form that relates downstream performance to upstream performance. \citet{Alabdulmohsi2022revisiting} proposed functional form $(y - \epsilon_{\infty}) / ((\epsilon_{0} - y)^a) = bx$ for relating scale to performance and released a scaling laws benchmark dataset that we use in section 

%\todo[inline]{NEED TO TALK ABOUT HOW EQUATION 6.1 OF SCALING LAWS FOR TRANSFER (plus a trivial constant for irreducible entropy) IS MATHEMATICALLY EQUIVALENT TO BNSL}

Smoothly broken power law functional forms equivalent to equation \ref{eq:UniversalScalingLaw} are common in the astrophysics literature (e.g. \cite{dampe2017direct}), but have not been used to fit scaling data in machine learning.
%\citet{2021arXiv210201293H}  - this has full list of authors/too long/not the format used in biblio for a conference
\citet{brown2020language}
described a smoothly broken power law functional form (consisting of 5 constants after reducing redundant variables) in equation 6.1 of their paper to relate scale and downstream performance. 
This is mathematically equivalent to our BNSL with a single break; however: (i) they proposed it only in the specific context of how fine-tuning plus transfer learning scales as a function of the model size. Their functional form contains a break only with respect to the number of model parameters but not with the dataset size; (ii) they only mentioned this equation in passing and do not attempt to fit any data using this functional form; (iii) they arrived at it simply via combining the scaling law for transfer that is the focus of their work with a scaling law for pretraining data, (iv) they did not identify it as a smoothly broken power law, or note any qualitative advantages of this functional form. (v) they do not talk about the family of functional forms with multiple breaks. 

%but to the best of our knowledge have never been mentioned or utilized in any literature that involves artificial neural networks.


TODO: Maybe mention "Limits of Large-Scale Training" Function
%TODO: mention that \citet{DBLP:journals/corr/abs-1909-12673} attempts to model transition from random guessing to power law
%TODO: explain why a,b,c,d are all non-negative.


==> old__not_used_anymore/sections_ir/sec_theory.tex <==
\section{Theoretical Limitations of Other Scaling Laws}

%\todo[inline]{I'm not sure it's worth including any propositions in the main text.  The proofs are just basic calculus and algebra.}


%\todo[inline]{This is for M2.  Need to do M3 (and maybe M4) case as well.  Also need to know which one(s) to consider "standard" for framing.}

Our use of BNSLs is inspired by the observation that scaling is not always well predicted by a simple power law.
Nor are the modifications which have been applied in previous works sufficient to capture the qualitative properties of empirical scaling curves.  
In effect, the most sophisticated form common in previous work is a power law modified to incorporate a minimum achievable loss, representing irreducible entropy, and TODO.
Here we show mathematically two qualitative defects of these functional forms:
\begin{enumerate}
    \item They are strictly monotonic and thus unable to fit double descent phenomena.
    \item They cannot express inflection points, which are frequently observed empirically.
\end{enumerate}
%This can be seen by observing that thes
Note that these functional forms \textit{can} exhibit inflection points on the log-log axes which are commonly used for plotting scaling data.  
However, on a linear-linear plot, the extra expressiveness of broken neural scaling laws is required (and sufficient).
Figure~\ref{fig:double_descent} and Figure~\ref{fig:arithmetic}, provides examples of BNSLs (with a single break-point, $n=1$) producing double descent and inflection points, respectively, establishing the capacity of this functional form to fit these phenomena.

We now explain why standard functional forms are incapable of exhibiting either behavior.
First, recall that expressions of the form $m^n$ can only take the value $0$ if $m=0$. 
We now examine the expressions for the first and second derivatives of M1, M2, M3, M3', provided in Table~\ref{tab:math}, and observe that they are all continuous and do not have roots over the relevant ranges of $a,b,c,d,x>0$, $b<1$.
This implies that they are monotonic (as the first derivative never changes sign), and that they lack inflection points (since an inflection point must have $f''(x)=0$).

\begin{table}[h]
\centering
\begin{tabular}{c|c|c|c}
name & $f(x)$ & $f'(x)$ & $f''(x)$ \\
\midrule
M1  & $ax^b$ & $abx^{b-1}$ & $ab(b-1)x^{b-2}$ \\
\midrule
M2  & $ax^b + c$ & $abx^{b-1}$ & $ab(b-1)x^{b-2}$ \\
%M2  & $f(x)$ & $f'(x)$ & $\frac{(c (1 + c) (b/x)^c)}{x^2}$ \\
\midrule
M3  & $a(x^{-1} + d)^{-b} + c$  & 
%$\frac{a b }{x (1 + d x)(d + 1/x)^{b}}$  & $a b x^{(b-2)} (1 + d x)^{(-2 - b)} (b -1 - 2 d x) $ \\
$a b  x^{(b-1)} (1 + d x)^{(-1 - b)}$  & $a b x^{(b-2)} (1 + d x)^{(-2 - b)} (b -1 - 2 d x) $ 
% \midrule
% M3' & $f(x)$ & $f'(x)$ & $f''(x)$ \\
%The above expression does not have a root for $a,b,d,x>0; b < 1$: the first two terms are strictly positive, meaning we would need $b = 2dx + 1 \geq 1$.
\label{tab:math}
\end{tabular}
\caption{
    Previously proposed functional forms and their (first and second order) derivatives.  
    For $a,b,c,d,x>0$, $b<1$, the expressions for each of the derivatives is a product of non-zero multiplicands, and thus none of these functional forms can express functions that are non-monotonic or have inflection points.
    %The above expression does not have a root for $a,b,d,x>0; b < 1$: the first two terms are strictly positive, meaning we would need $b = 2dx + 1 \geq 1$.
 }
\end{table}


Figure \ref{fig:Inflection_Point_example} is an example of this inflection point present in experimental data from a real world downstream task, Two Digit Addition (Zero-Shot) from \citet{brown2020language}. %\citet{2020arXiv200514165B}. 
In the small scale regime, the function is concave downward as it transitions from random guessing performance to starting to learn the task. As the scale increases past the small scale regime, an inflection point is reached and the function becomes concave upward as power law scaling behaviour takes over.



% % M3: (need d>0) 
% M3: $f(x) = a(x^{-1} + d)^{-b} + c$ 
% $$
%  f'(x) = \frac{a b }{x (1 + d x)(d + 1/x)^{b}} 
% $$
% $$
%  f''(x) = a b x^{(b-2)} (1 + d x)^{(-2 - b)} (b -1 - 2 d x) 
% $$
% The above expression does not have a root for $a,b,d,x>0; b < 1$: the first two terms are strictly positive, meaning we would need $b = 2dx + 1 \geq 1$.

% "also M3?": $f(x)=a(x+d)^b + c$
% $$
% f'(x) = a b (d + x)^{(b-1)}
% $$
% $$
% f''(x) = a (-1 + b) b (d + x)^{(b-2)}
% $$
% Neither of the above expressions have roots because they are a product of non-zero constants and expressions of the form $m^n$.


%M2: $y = ax^b +c$


% \subsection{SCRAPS}

% % TODO: convert this to same form as M2
% \begin{proposition}
%     Functions of the form $f(x) = a + \left(\frac{b}{x}\right)^c$ are necessarily monotonic for $a,b,c>0$ in the range $x>0$.
% \end{proposition}
% \begin{proof}
%     A sufficient condition for monotonicity is that $f'(x)$ does not change sign.  
%     In our case, we have 
%     $$
%     f'(x) = - bc \left(\frac{b}{x}\right)^{(c-1)}.
%     $$
%     Since $b$ and $x$ are both positive, so is the ratio $\frac{b}{x}$.  
%     And since a positive number taken to any power is also positive, the entire expression is guaranteed to be negative for all values of $a,b,c,x>0$.
% \end{proof}

% %TODO: rename this section to "Math Proofs" and also prove that other functional forms can't express non-monotonic behavior

% \begin{proposition}
%     Functions of the form $f(x) = a + \left(\frac{b}{x}\right)^c$ cannot contain an inflection point for $a,b,c>0$ in the range $x>0$.
% \end{proposition}
% \begin{proof}
% The second derivative is:
% $$
% f''(x) = 
% \frac{(c (1 + c) (b/x)^c)}{x^2}.
% $$
% Since $b$, $c$ and $x$ are all positive, all of the multiplicands of $f''(x)$ are positive, and thus so is $f''(x)$, but an inflection point must have $f''(x)=0$.
% \end{proof}

% \subsection{SCRAPS}

% An inflection point is a point of a curve at which the second order derivative (i.e.\ curvature) changes signs. 
% Empirically, the function relating the performance evaluation metric (e.g. prediction error) to the quantity being scaled (e.g.\ model size) often has an inflection point. 
% Figure \ref{fig:Inflection_Point_example} is an example of this inflection point present in experimental data from a real world downstream task, Two Digit Addition (Zero-Shot) from \citet{brown2020language}. %\citet{2020arXiv200514165B}. 
% In the small scale regime, the function is concave downward as it transitions from random guessing performance to starting to learn the task. 
% As the scale increases past the small scale regime, an inflection point is reached and the function becomes concave upward as power law scaling behaviour takes over.

% However, \textbf{Proposition:} typical functional form cannot have an inflection point.
% \textbf{Proof:}
% %https://www.wolframalpha.com/input?i=d%5E2%2Fdx%5E2+%28a+%2B+%28b%2Fx%29**c%29+
% An inflection point is a point of a curve at which the second order derivative (i.e.\ curvature) changes signs. 
% The second derivative of this function is:
% $$
% f''(x) = 
% \frac{(c (1 + c) (b/x)^c)}{x^2}.
% $$
% Since $b$, $c$ and $x$ are all positive, all of the multiplicands of $f''(x)$ are positive, and thus so is $f''(x)$, but an inflection point must have $f''(x)=0$.
% % https://www.wolframalpha.com/input?i=d%5E2%2Fdx%5E2+%28a+%2B+%28b%2Fx%29**c+%281+%2F+%28x%2Bd%29%5Ef%29%29

% Note that inflection points often appear in scaling curves, which are typically plotted on log/log axes, and existing scaling laws can fit those inflection points (TODO: is this right?  I thought they were just linear on a log/log plot?).
% Inflection points are less common but still sometimes present in a linear/linear plot; These are the inflection points that existing scaling laws cannot capture.

% TODO: do we get the same result for all of M1 through M4?

% All the functional forms:

% M1: $y = ax^b$

% M2: $y = ax^b +c$

% M3: $y = a(x^{-1} + d)^{-b} + c$ 

% also M3?: $y=a(x+d)^b + c$

% M4: $(y - \epsilon_{\infty}) / ((\epsilon_{0} - y)^a) = bx$ 

% $\epsilon_{\infty}$ is irreducible loss, and $\epsilon_{0}$ is performance of random guessing.

% Equation 6.1 of "scaling laws for transfer" paper: $y = (ax^b + cx^d)^f + g$

% I (Ethan) just now have realized that this equation 6.1 above is a smoothly broken power law (i.e. mathematically equivalent to ours I think) too so we have to change the narrative of the paper now:  
% \url{https://math.stackexchange.com/a/2427151}

% \url{https://colab.research.google.com/drive/1QP81soNf1DDV_Q6iimN8sb-hZHaZeMyW}

% Also, I think "scaling laws for transfer" paper may/might have been unaware that its equation 6.1 is a thing called a smoothly broken power law.

% Broken Neural Scaling Law: $y =  a + \left(\frac{b}{x}\right)^c \prod_{i=1}^n \left(1 + \left(\frac{x}{d_i}\right)^{f_i}\right)^{-g_i}$



% TODO: remove this section?
% TODO: replace it with section about breaks rather than inflection points


%This inflection point at the transition from constant random guessing performance in the small scale regime to 
%When the performance evaluation metric (e.g. prediction error) is plotted on y-axis and the quantity being scaled (e.g. model size) is plotted on x-axis, the plotted data has an inflection point at the transition from constant random guessing performance in the small scale regime to 
% Figure \ref{fig:Inflection_Point_example} is an example of this inflection point present in experimental data from a real world downstream task, Two Digit Addition (Zero-Shot) from \citet{brown2020language}. %\citet{2020arXiv200514165B}. 
%In the small scale regime, the function is concave downward as it transitions from random guessing performance to starting to learn the task. As the scale increases past the small scale regime, an inflection point is reached and the function becomes concave upward as power law scaling behaviour takes over.

% \todo[inline]{math proofs}

% 1. proof that shows $y=a/(x^b+d)+c$ has inflection point for all functions in which $a$ $!=0$, $b>1$, and $d>0$ are simultaneously true

% 2. proof that shows $y=a(x+d)^b + c$ never has inflection point
